The Planck clusters in the LOFAR sky. I. LoTSS-DR2: new detections and sample overview

Relativistic electrons and magnetic fields permeate the intra-cluster medium (ICM) and manifest themselves as diffuse sources of synchrotron emission observable at radio wavelengths, namely radio halos and radio relics. Although there is broad consensus that the formation of these sources is connected to turbulence and shocks in the ICM, the details of the required particle acceleration, the strength and morphology of the magnetic field in the cluster volume, and the influence of other sources of high-energy particles are poorly known. Sufficiently large samples of radio halos and relics, which would allow us to examine the variation among the source population and pinpoint their commonalities and differences, are still missing. At present, large numbers of these sources are easiest to detect at low radio frequencies, where they shine brightly. We examined the low-frequency radio emission from all 309 clusters in the second catalog of Planck Sunyaev Zel'dovich detected sources that lie within the 5634 deg$^2$ covered by the Second Data Release of the LOFAR Two-meter Sky Survey (LoTSS-DR2). We produced LOFAR images at different resolutions, with and without discrete sources subtracted, and created overlays with optical and X-ray images before classifying the diffuse sources in the ICM, guided by a decision tree. Overall, we found 83 clusters that host a radio halo and 26 that host one or more radio relics (including candidates). About half of them are new discoveries. The detection rate of clusters hosting a radio halo and one or more relics in our sample is $30\pm11$% and $10\pm6$%, respectively. Extrapolating these numbers, we anticipate that once LoTSS covers the entire northern sky it will provide the detection of $251\pm92$ clusters hosting a halo and $83\pm50$ clusters hosting at least one relic from Planck clusters alone.

==> tables/table_RH_sample.tex <==
PSZ2 G023.17+86.71 & 25.73 & 3.12 & 29.84 & 3.62 & 9.76e+24 & 1.18e+24 & 5.79 & 0.34 & 232.8 & 11.7 & 95.1 & 6.4 & rotated\_ellipse & 19.81 & 0.347 & 1.18 & --- \\
PSZ2 G031.93+78.71 & 189.84 & 78.34 & 176.45 & 78.03 & 2.28e+24 & 1.01e+24 & 11.39 & 0.20 & 78.7 & 1.1 &  &  & circle & 66.26 & 0.168 & 3.27 & --- \\
PSZ2 G040.58+77.12 & 50.33 & 6.76 & 42.92 & 7.82 & 6.04e+23 & 1.10e+23 & 0.67 & 0.10 & 165.3 & 21.0 &  &  & circle & 7.01 & 0.082 & 2.46 & --- \\
PSZ2 G045.87+57.70 & 10.78 & 2.59 & 11.75 & 2.79 & 2.11e+25 & 5.03e+24 & 14.18 & 1.90 & 89.0 & 9.6 &  &  & circle & 9.66 & 0.877 & 1.11 & --- \\
PSZ2 G046.88+56.48 & 177.19 & 20.99 & 236.45 & 27.77 & 8.36e+24 & 9.81e+23 & 1.57 & 0.07 & 369.9 & 13.6 &  &  & circle & 22.46 & 0.131 & 0.70 & --- \\
PSZ2 G048.10+57.16 & 300.00 & 39.36 & 354.88 & 44.67 & 5.43e+24 & 6.84e+23 & 1.58 & 0.05 & 463.4 & 15.6 & 220.7 & 6.3 & rotated\_ellipse & 32.61 & 0.160 & 0.87 & --- \\
PSZ2 G049.32+44.37 & 45.87 & 7.71 & 70.64 & 10.61 & 1.73e+24 & 2.59e+23 & 0.61 & 0.05 & 281.2 & 19.7 &  &  & circle & 12.13 & 0.099 & 0.79 & --- \\
PSZ2 G053.53+59.52 & 519.08 & 57.38 & 387.17 & 45.84 & 1.32e+25 & 1.56e+24 & 11.66 & 0.11 & 171.5 & 1.4 &  &  & circle & 104.71 & 0.141 & 13.68 & --- \\
PSZ2 G055.59+31.85 & 30.25 & 5.21 & 33.57 & 5.46 & 5.29e+24 & 8.60e+23 & 17.48 & 0.71 & 72.3 & 2.3 &  &  & circle & 30.72 & 0.433 & 1.26 & --- \\
PSZ2 G056.77+36.32 & 79.79 & 26.53 & 83.39 & 26.97 & 1.95e+24 & 6.30e+23 & 1.10 & 0.10 & 223.3 & 15.5 &  &  & circle & 14.15 & 0.099 & 0.79 & --- \\
PSZ2 G063.38+53.44 & 27.53 & 5.02 & 29.40 & 5.19 & 2.09e+25 & 3.70e+24 & 10.76 & 0.58 & 133.0 & 5.8 &  &  & circle & 20.38 & 0.713 & 1.08 & --- \\
PSZ2 G066.34+26.14 & 98.35 & 12.89 & 82.29 & 11.71 & 1.55e+26 & 2.20e+25 & 22.02 & 0.70 & 190.5 & 5.1 &  &  & circle & 32.77 & 1.304 & 1.60 & --- \\
PSZ2 G066.41+27.03 & 89.88 & 10.47 & 111.34 & 12.61 & 1.72e+26 & 1.95e+25 & 15.50 & 0.42 & 374.5 & 11.0 & 173.6 & 5.1 & rotated\_ellipse & 36.36 & 1.096 & 1.05 & --- \\
PSZ2 G069.39+68.05 & 14.60 & 2.46 & 18.49 & 4.42 & 5.86e+25 & 1.40e+25 & 4.73 & 1.01 & 211.9 & 38.5 &  &  & circle & 4.64 & 0.826 & 0.71 & --- \\
PSZ2 G071.21+28.86 & 45.99 & 7.74 & 67.70 & 10.82 & 3.41e+25 & 5.44e+24 & 1.53 & 0.13 & 490.3 & 35.6 &  &  & circle & 11.08 & 0.260 & 1.32 & --- \\
PSZ2 G080.70+48.31 & 8.18 & 2.89 & 6.39 & 2.86 & 1.12e+24 & 5.03e+23 & 4.58 & 0.65 & 64.1 & 6.5 &  &  & circle & 8.75 & 0.324 & 0.96 & --- \\
PSZ2 G081.02+50.57 & 5.39 & 1.08 & 10.59 & 2.09 & 1.15e+25 & 2.28e+24 & 1.45 & 0.33 & 238.3 & 36.7 &  &  & circle & 6.46 & 0.175 & 0.87 & --- \\
PSZ2 G083.29-31.03 & 53.22 & 5.88 & 54.71 & 6.00 & 3.67e+25 & 4.03e+24 & 6.71 & 0.28 & 226.5 & 7.8 &  &  & circle & 26.25 & 0.341 & 1.65 & --- \\
PSZ2 G084.10+58.72 & 3.80 & 0.85 & 3.97 & 0.96 & 1.13e+25 & 2.74e+24 & 6.03 & 1.79 & 85.5 & 17.5 &  &  & circle & 6.49 & 0.320 & 1.05 & --- \\
PSZ2 G084.13-35.41 & 51.57 & 13.14 & 56.55 & 13.48 & 1.97e+25 & 4.69e+24 & 6.16 & 0.31 & 201.8 & 8.4 &  &  & circle & 20.03 & 0.565 & 1.17 & --- \\
PSZ2 G085.23+39.42 & 55.35 & 7.81 & 68.62 & 8.84 & 1.49e+25 & 1.92e+24 & 5.12 & 0.18 & 211.5 & 4.8 &  &  & circle & 40.12 & 0.262 & 1.80 & --- \\
PSZ2 G086.93+53.18 & 8.91 & 1.69 & 11.50 & 2.20 & 2.67e+25 & 5.09e+24 & 3.29 & 0.54 & 190.7 & 25.2 &  &  & circle & 7.29 & 0.486 & 1.02 & --- \\
PSZ2 G089.39+69.36 & 11.77 & 2.17 & 10.93 & 2.14 & 2.58e+25 & 5.05e+24 & 10.47 & 0.79 & 104.6 & 6.2 &  &  & circle & 16.23 & 0.532 & 0.83 & --- \\
PSZ2 G096.83+52.49 & 39.63 & 7.45 & 45.21 & 7.80 & 1.62e+25 & 2.80e+24 & 7.92 & 0.23 & 211.0 & 5.9 & 122.2 & 3.9 & rotated\_ellipse & 36.70 & 0.417 & 1.53 & --- \\
PSZ2 G097.72+38.12 & 152.51 & 16.07 & 140.24 & 14.94 & 1.19e+25 & 1.27e+24 & 7.44 & 0.14 & 183.2 & 2.9 &  &  & circle & 55.12 & 0.276 & 1.26 & --- \\
PSZ2 G098.30-41.15 & 46.52 & 7.17 & 42.00 & 6.87 & 3.24e+25 & 5.31e+24 & 40.22 & 1.10 & 83.8 & 1.7 &  &  & circle & 44.54 & 0.746 & 2.24 & --- \\
PSZ2 G099.86+58.45 & 21.92 & 4.82 & 19.92 & 4.74 & 3.87e+25 & 9.21e+24 & 7.36 & 0.49 & 163.2 & 8.6 &  &  & circle & 15.69 & 0.687 & 1.10 & --- \\
PSZ2 G100.96-24.07 & 17.18 & 7.03 & 18.45 & 7.24 & 1.33e+25 & 5.21e+24 & 5.82 & 0.75 & 143.7 & 14.6 &  &  & circle & 8.78 & 0.544 & 0.95 & --- \\
PSZ2 G106.61+66.71 & 19.45 & 2.41 & 17.91 & 2.27 & 7.07e+24 & 8.98e+23 & 12.82 & 0.52 & 81.7 & 2.5 &  &  & circle & 32.54 & 0.257 & 1.97 & --- \\
PSZ2 G107.10+65.32 & 270.18 & 36.21 & 154.77 & 29.94 & 7.16e+25 & 9.60e+24 & 22.66 & 1.44 & 251.1 & 16.0 & 102.9 & 7.0 & rotated\_ellipse & 17.21 & 0.253 & 2.87 & $P_{150}$ derived from $S_{150}$ ($2\sigma$) \\
PSZ2 G108.27+48.66 & 10.26 & 3.30 & 9.39 & 3.23 & 2.17e+25 & 7.47e+24 & 6.42 & 0.84 & 123.3 & 12.0 &  &  & circle & 9.63 & 0.563 & 0.94 & --- \\
PSZ2 G109.97+52.84 & 13.61 & 1.91 & 16.25 & 2.58 & 6.18e+24 & 9.80e+23 & 1.39 & 0.16 & 233.5 & 25.0 &  &  & circle & 9.07 & 0.127 & 1.95 & --- \\
PSZ2 G111.75+70.37 & 28.12 & 20.02 & 29.28 & 20.05 & 2.90e+24 & 1.99e+24 & 2.53 & 0.14 & 218.1 & 12.9 & 105.7 & 6.5 & rotated\_ellipse & 20.34 & 0.149 & 1.49 & --- \\
PSZ2 G112.48+56.99 & 41.72 & 7.00 & 55.16 & 8.36 & 6.71e+23 & 1.02e+23 & 0.80 & 0.05 & 160.7 & 9.3 &  &  & circle & 16.05 & 0.071 & 1.00 & --- \\
PSZ2 G113.91-37.01 & 78.03 & 8.22 & 122.78 & 13.64 & 6.38e+25 & 7.09e+24 & 5.09 & 0.23 & 365.3 & 15.0 &  &  & circle & 20.92 & 0.786 & 1.47 & --- \\
PSZ2 G114.31+64.89 & 41.10 & 11.72 & 66.61 & 13.27 & 1.83e+25 & 3.64e+24 & 12.40 & 0.59 & 143.9 & 6.6 &  &  & circle & 19.50 & 0.369 & 1.67 & --- \\
PSZ2 G115.67-27.57 & 4.61 & 0.84 & 4.53 & 0.74 & 3.93e+24 & 6.39e+23 & 5.00 & 1.33 & 80.3 & 14.0 &  &  & circle & 7.86 & 0.287 & 0.93 & --- \\
PSZ2 G133.60+69.04 & 145.00 & 18.87 & 162.80 & 20.30 & 3.43e+25 & 4.28e+24 & 7.07 & 0.17 & 377.1 & 5.2 & 200.9 & 4.3 & rotated\_ellipse & 74.85 & 0.248 & 3.13 & --- \\
PSZ2 G135.17+65.43 & 35.76 & 6.89 & 40.76 & 7.35 & 5.46e+25 & 9.84e+24 & 6.43 & 0.50 & 232.7 & 12.1 &  &  & circle & 19.65 & 0.576 & 1.24 & --- \\
PSZ2 G138.32-39.82 & 28.07 & 4.29 & 31.00 & 4.80 & 8.22e+24 & 1.27e+24 & 2.89 & 0.24 & 201.7 & 14.3 &  &  & circle & 12.23 & 0.419 & 1.07 & --- \\
PSZ2 G139.18+56.37 & 398.78 & 49.86 & 288.44 & 41.53 & 1.47e+26 & 1.84e+25 & 45.75 & 0.25 & 170.2 & 0.8 &  &  & circle & 195.52 & 0.369 & 20.10 & $P_{150}$ derived from $S_{150}$ ($2\sigma$) \\
PSZ2 G141.05-32.61 & 66.30 & 8.94 & 71.57 & 9.78 & 1.00e+26 & 1.37e+25 & 6.30 & 0.32 & 314.6 & 12.8 &  &  & circle & 19.40 & 0.525 & 1.68 & --- \\
PSZ2 G143.26+65.24 & 33.72 & 4.79 & 34.02 & 5.12 & 1.68e+25 & 2.53e+24 & 4.30 & 0.27 & 206.5 & 11.7 &  &  & circle & 16.23 & 0.389 & 1.07 & --- \\
PSZ2 G144.23-18.19 & 17.33 & 3.12 & 23.80 & 3.96 & 2.10e+24 & 3.79e+23 & 1.80 & 0.18 & 174.2 & 15.0 &  &  & circle & 11.02 & 0.214 & 1.05 & $P_{150}$ and $r_1$ computed assuming $z=0.2$ \\
PSZ2 G147.88+53.24 & 12.90 & 3.63 & 21.86 & 4.27 & 3.75e+25 & 7.33e+24 & 5.87 & 0.38 & 187.0 & 10.9 &  &  & circle & 14.18 & 0.595 & 1.03 & --- \\
PSZ2 G148.36+75.23 & 20.97 & 2.33 & 18.86 & 2.16 & 6.07e+24 & 6.95e+23 & 8.57 & 0.58 & 96.6 & 5.1 &  &  & circle & 18.46 & 0.343 & 1.00 & --- \\
PSZ2 G149.22+54.18 & 332.74 & 52.81 & 315.77 & 51.81 & 1.64e+25 & 2.69e+24 & 6.42 & 0.11 & 246.1 & 3.6 &  &  & circle & 56.88 & 0.234 & 2.07 & --- \\
PSZ2 G149.75+34.68 & 711.34 & 74.64 & 574.12 & 61.67 & 5.62e+25 & 6.04e+24 & 12.23 & 0.08 & 303.9 & 1.6 &  &  & circle & 157.82 & 0.184 & 7.23 & --- \\
PSZ2 G150.56+46.67 & 13.87 & 1.58 & 16.18 & 1.88 & 9.98e+24 & 1.16e+24 & 4.17 & 0.26 & 153.0 & 7.6 &  &  & circle & 17.50 & 0.388 & 0.96 & --- \\
PSZ2 G150.56+58.32 & 54.22 & 11.09 & 60.83 & 11.53 & 5.65e+25 & 1.07e+25 & 10.66 & 0.37 & 315.3 & 11.2 & 132.6 & 4.8 & rotated\_ellipse & 29.55 & 0.607 & 1.22 & --- \\
PSZ2 G151.19+48.27 & 38.62 & 7.69 & 47.05 & 9.01 & 1.34e+25 & 2.57e+24 & 1.66 & 0.13 & 335.5 & 23.7 &  &  & circle & 11.15 & 0.202 & 0.95 & --- \\
PSZ2 G154.13+40.19 & 13.50 & 1.82 & 13.20 & 1.83 & 3.80e+24 & 5.26e+23 & 9.04 & 0.64 & 76.2 & 4.1 &  &  & circle & 17.60 & 0.422 & 0.89 & --- \\
PSZ2 G156.26+59.64 & 6.59 & 1.65 & 7.81 & 1.97 & 1.27e+25 & 3.22e+24 & 9.74 & 1.90 & 85.9 & 13.7 &  &  & circle & 6.48 & 0.948 & 0.94 & --- \\
PSZ2 G160.83+81.66 & 11.67 & 2.70 & 10.56 & 2.67 & 4.98e+25 & 1.26e+25 & 15.90 & 1.26 & 91.7 & 5.5 &  &  & circle & 16.69 & 0.647 & 1.21 & --- \\
PSZ2 G164.65+46.37 & 23.52 & 5.28 & 22.40 & 5.29 & 9.56e+24 & 2.26e+24 & 5.87 & 0.33 & 217.1 & 12.0 & 87.5 & 5.4 & rotated\_ellipse & 18.86 & 0.413 & 0.89 & --- \\
PSZ2 G165.06+54.13 & 43.38 & 9.18 & 60.61 & 10.76 & 3.51e+24 & 6.23e+23 & 0.88 & 0.06 & 305.0 & 18.4 &  &  & circle & 14.18 & 0.108 & 0.76 & --- \\
PSZ2 G166.09+43.38 & 142.10 & 15.44 & 112.78 & 12.81 & 1.65e+25 & 1.87e+24 & 7.19 & 0.16 & 202.0 & 3.9 &  &  & circle & 46.32 & 0.210 & 1.39 & --- \\
PSZ2 G166.62+42.13 &  &  &  &  &  &  &  &  &  &  &  &  & --- &  &  &  & Cannot be disentangled from RR emission \\
PSZ2 G172.63+35.15 & 56.64 & 7.29 & 68.09 & 9.27 & 2.99e+24 & 4.07e+23 & 1.79 & 0.16 & 202.5 & 15.1 &  &  & circle & 12.26 & 0.172 & 1.02 & --- \\
PSZ2 G176.27+37.54 & 4.73 & 1.11 & 6.47 & 2.12 & 9.62e+24 & 3.16e+24 & 2.96 & 1.05 & 139.6 & 40.7 &  &  & circle & 3.47 & 0.375 & 1.10 & --- \\
PSZ2 G179.09+60.12 & 25.21 & 6.99 & 36.51 & 8.04 & 1.89e+24 & 4.17e+23 & 2.55 & 0.22 & 133.0 & 10.4 &  &  & circle & 11.31 & 0.293 & 1.27 & --- \\
PSZ2 G183.30+34.98 & 24.35 & 7.35 & 32.35 & 8.01 & 1.92e+25 & 4.76e+24 & 5.65 & 0.49 & 184.1 & 13.8 &  &  & circle & 11.63 & 0.761 & 0.92 & --- \\
PSZ2 G183.90+42.99 & 57.09 & 5.92 & 52.12 & 5.40 & 7.55e+25 & 7.81e+24 & 16.35 & 0.39 & 167.6 & 3.1 &  &  & circle & 45.83 & 0.606 & 1.48 & --- \\
PSZ2 G184.68+28.91 & 7.03 & 1.23 & 6.86 & 1.41 & 1.94e+24 & 3.98e+23 & 5.40 & 0.93 & 70.7 & 9.8 &  &  & circle & 7.17 & 0.473 & 0.64 & --- \\
PSZ2 G186.37+37.26 & 88.01 & 9.11 & 85.31 & 9.04 & 2.30e+25 & 2.44e+24 & 12.40 & 0.43 & 162.2 & 4.8 &  &  & circle & 30.41 & 0.533 & 1.10 & --- \\
PSZ2 G186.61+62.94 & 3.10 & 1.10 & 3.21 & 1.11 & 3.64e+24 & 1.26e+24 & 2.85 & 0.82 & 94.9 & 18.6 &  &  & circle & 6.61 & 0.191 & 0.53 & --- \\
PSZ2 G186.99+38.65 & 54.29 & 7.14 & 55.06 & 7.28 & 3.00e+25 & 3.96e+24 & 27.68 & 0.90 & 106.1 & 2.8 &  &  & circle & 35.46 & 0.625 & 1.30 & --- \\
PSZ2 G189.31+59.24 & 334.87 & 68.03 & 252.77 & 64.40 & 1.09e+25 & 2.78e+24 & 25.80 & 0.39 & 102.3 & 1.2 &  &  & circle & 78.08 & 0.189 & 4.63 & --- \\
PSZ2 G190.61+66.46 & 17.61 & 2.44 & 35.59 & 4.35 & 3.63e+25 & 4.44e+24 & 3.22 & 0.23 & 290.5 & 15.0 &  &  & circle & 16.68 & 0.252 & 1.85 & --- \\
PSZ2 G192.18+56.12 & 14.92 & 2.52 & 19.45 & 3.59 & 8.10e+23 & 1.50e+23 & 0.66 & 0.10 & 174.9 & 22.1 &  &  & circle & 7.24 & 0.102 & 1.01 & --- \\
PSZ2 G192.77+33.14 & 108.18 & 14.63 & 118.30 & 18.72 & 7.10e+23 & 1.12e+23 & 0.54 & 0.06 & 211.7 & 20.8 &  &  & circle & 9.37 & 0.062 & 0.75 & --- \\
PSZ2 G192.90+29.63 & 21.71 & 3.05 & 33.96 & 5.14 & 1.64e+25 & 2.48e+24 & 2.91 & 0.29 & 249.5 & 21.1 &  &  & circle & 9.53 & 0.412 & 0.88 & --- \\
PSZ2 G205.90+73.76 & 45.01 & 6.79 & 36.67 & 6.28 & 3.01e+25 & 5.15e+24 & 34.30 & 1.53 & 103.3 & 4.7 & 71.7 & 3.1 & rotated\_ellipse & 27.79 & 0.763 & 0.72 & --- \\

==> tables/table_RR_sample.tex <==
PSZ2 G048.10+57.16 &  & 230.0114 & 30.5267 & 264.28 & 26.83 & 3.96e+24 & 4.02e+23 & 998 & 35 & 395 & 182 & 2940 & 1515 & 206 &  &  \\
PSZ2 G057.61+34.93 &  & 257.7043 & 34.5640 & 426.57 & 42.90 & 6.74e+24 & 6.77e+23 & 1361 & 44 & 450 & 167 & 5579 & 1269 & 176 &  &  \\
PSZ2 G069.39+68.05 &  & 215.4091 & 38.3299 & 28.47 & 4.58 & 7.61e+25 & 1.22e+25 & 1489 & 56 & 109 & 153 & 1237 &  &  &  &  \\
PSZ2 G071.21+28.86 & N & 268.0816 & 44.7043 & 518.11 & 51.83 & 2.37e+26 & 2.37e+25 & 1254 & 39 & 291 & 149 & 6205 & 998 & 42 & 1941 & 39 \\
PSZ2 G071.21+28.86 & S & 267.9735 & 44.6313 & 179.66 & 17.99 & 8.23e+25 & 8.24e+24 & 813 & 39 & 136 & 86 & 5134 & 965 & 42 & 1941 & 39 \\
PSZ2 G080.16+57.65 &  & 225.5644 & 47.1942 & 37.63 & 4.78 & 7.27e+23 & 9.24e+22 & 1073 & 50 & 173 & 86 & 1667 & 1418 & 196 &  &  \\
PSZ2 G086.58+73.11 &  & 205.9581 & 39.9924 & 4.28 & 0.66 & 6.22e+23 & 9.53e+22 & 394 & 44 & 121 & 42 & 584 &  &  &  &  \\
PSZ2 G089.52+62.34 & N2 & 215.8002 & 48.7878 & 92.49 & 9.94 & 1.10e+24 & 1.19e+23 & 1213 & 35 & 296 & 200 & 2742 & 1721 & 233 &  &  \\
PSZ2 G089.52+62.34 & N1 & 215.5888 & 48.5719 & 50.64 & 6.63 & 6.04e+23 & 7.90e+22 & 273 & 35 & 107 & 39 & 5147 & 484 & 74 &  &  \\
PSZ2 G091.79-27.00 &  & 341.3831 & 28.2727 & 16.48 & 2.55 & 7.36e+24 & 1.14e+24 & 1535 & 41 & 164 & 96 & 1176 & 2510 & 339 &  &  \\
PSZ2 G096.43-20.89 &  & 341.9545 & 35.5495 & 33.56 & 4.16 & 1.38e+25 & 1.71e+24 & 1482 & 53 & 279 & 173 & 839 &  &  &  &  \\
PSZ2 G099.48+55.60 & N & 216.8435 & 57.0057 & 108.16 & 11.44 & 3.04e+24 & 3.22e+23 & 1711 & 45 & 354 & 173 & 1398 & 1366 & 49 & 2405 & 45 \\
PSZ2 G099.48+55.60 & S & 217.2878 & 56.7582 & 69.38 & 7.49 & 1.95e+24 & 2.11e+23 & 1090 & 45 & 229 & 160 & 1609 & 1068 & 48 & 2405 & 45 \\
PSZ2 G107.10+65.32 &  & 203.2562 & 50.4015 & 21.49 & 2.25 & 5.29e+24 & 5.53e+23 & 538 & 50 & 266 & 113 & 1258 & 1211 & 170 &  &  \\
PSZ2 G109.22-44.01 &  & 2.6228 & 17.7278 & 148.71 & 15.75 & 1.24e+25 & 1.31e+24 & 1168 & 40 & 211 & 100 & 3216 &  &  &  &  \\
PSZ2 G111.75+70.37 &  & 198.3618 & 46.3271 & 120.37 & 12.07 & 1.14e+25 & 1.14e+24 & 874 & 56 & 317 & 93 & 4520 & 898 & 133 &  &  \\
PSZ2 G113.91-37.01 & N & 4.9365 & 25.3543 & 164.61 & 16.57 & 7.78e+25 & 7.84e+24 & 1172 & 43 & 412 & 155 & 2033 & 1210 & 47 & 2605 & 43 \\
PSZ2 G113.91-37.01 & S & 4.8569 & 25.2329 & 40.41 & 4.43 & 1.91e+25 & 2.10e+24 & 1481 & 43 & 296 & 128 & 1361 & 1464 & 49 & 2605 & 43 \\
PSZ2 G116.50-44.47 &  & 8.0645 & 18.1766 & 13.00 & 1.54 & 7.17e+24 & 8.48e+23 & 555 & 47 & 118 & 79 & 946 & 890 & 128 &  &  \\
PSZ2 G121.03+57.02 &  & 194.9253 & 60.0416 & 12.26 & 1.57 & 4.86e+24 & 6.21e+23 & 542 & 44 & 141 & 45 & 759 & 570 & 88 &  &  \\
PSZ2 G135.17+65.43 &  & 184.7975 & 50.8694 & 6.61 & 0.93 & 7.78e+24 & 1.10e+24 & 654 & 54 & 125 & 63 & 552 & 1110 & 158 &  &  \\
PSZ2 G144.99-24.64 &  & 37.2926 & 33.9827 & 10.45 & 2.12 & 1.07e+24 & 2.18e+23 & 773 & 48 & 153 & 82 & 749 &  &  &  &  \\
PSZ2 G151.19+48.27 &  & 154.4696 & 59.5328 & 19.24 & 2.05 & 5.09e+24 & 5.44e+23 & 812 & 43 & 122 & 90 & 816 & 682 & 101 &  &  \\
PSZ2 G165.46+66.15 & N & 170.8381 & 43.1768 & 89.07 & 9.43 & 9.79e+24 & 1.04e+24 & 1069 & 49 & 339 & 120 & 2270 & 843 & 51 & 2115 & 49 \\
PSZ2 G165.46+66.15 & S & 170.9279 & 43.0079 & 171.63 & 17.51 & 1.89e+25 & 1.92e+24 & 1638 & 49 & 385 & 188 & 2571 & 1387 & 53 & 2115 & 49 \\
PSZ2 G166.62+42.13 & W & 137.2336 & 51.5893 & 454.39 & 45.53 & 7.29e+25 & 7.30e+24 & 1901 & 39 & 718 & 238 & 2529 & 1462 & 200 &  &  \\
PSZ2 G166.62+42.13 & N & 137.4405 & 51.6072 & 32.37 & 3.67 & 5.19e+24 & 5.88e+23 & 932 & 39 & 364 & 163 & 675 & 917 & 129 &  &  \\
PSZ2 G166.62+42.13 & E & 137.5390 & 51.5332 & 12.21 & 6.52 & 1.96e+24 & 1.05e+24 & 1100 & 39 & 148 & 71 & 1080 & 1204 & 166 &  &  \\
PSZ2 G181.06+48.47 & N & 144.9131 & 40.8741 & 28.22 & 2.98 & 4.89e+24 & 5.17e+23 & 1394 & 39 & 135 & 67 & 925 & 1660 & 47 & 2694 & 39 \\
PSZ2 G181.06+48.47 & S & 144.8281 & 40.6879 & 66.76 & 6.83 & 1.16e+25 & 1.18e+24 & 1660 & 39 & 207 & 122 & 1083 & 1035 & 42 & 2694 & 39 \\
PSZ2 G186.99+38.65 &  & 132.5838 & 36.1125 & 12.42 & 1.58 & 6.14e+24 & 7.80e+23 & 723 & 46 & 136 & 73 & 705 & 1030 & 145 &  &  \\
PSZ2 G190.61+66.46 &  & 166.5720 & 33.5517 & 60.49 & 6.43 & 5.48e+25 & 5.82e+24 & 573 & 48 & 184 & 180 & 2331 & 865 & 126 &  &  \\
PSZ2 G198.46+46.01 &  & 142.7257 & 28.7635 & 41.68 & 4.64 & 1.19e+25 & 1.33e+24 & 1494 & 43 & 247 & 172 & 694 &  &  &  &  \\
PSZ2 G205.90+73.76 & N & 174.5111 & 27.9806 & 5.37 & 0.97 & 3.95e+24 & 7.12e+23 & 664 & 48 & 125 & 42 & 791 & 1490 & 53 & 2958 & 48 \\
PSZ2 G205.90+73.76 & S & 174.5439 & 27.8404 & 7.55 & 1.12 & 5.55e+24 & 8.26e+23 & 655 & 48 & 155 & 58 & 1028 & 1540 & 54 & 2958 & 48 \\

==> tables/table_asteriskRH_sample.tex <==
PSZ2 G071.39+59.54 & 20.01 & 2.30 & 88.87 & 11.90 & 2.60e+25 & 3.48e+24 & 1.27 & 0.08 & 529.2 & 36.0 & circle & 11.25 & 0.319 & 1.15 \\
PSZ2 G076.55+60.29 & 8.14 & 1.67 & 22.52 & 5.72 & 6.33e+24 & 1.61e+24 & 0.43 & 0.07 & 453.8 & 82.3 & circle & 4.40 & 0.118 & 0.76 \\
PSZ2 G077.90-26.63 & 28.02 & 4.04 & 64.10 & 10.75 & 3.89e+24 & 6.52e+23 & 1.88 & 0.24 & 218.1 & 26.5 & circle & 7.53 & 0.439 & 1.03 \\
PSZ2 G095.29+44.13 & 13.82 & 2.08 & 27.38 & 4.36 & 1.08e+25 & 1.72e+24 & 1.21 & 0.13 & 328.7 & 32.8 & circle & 8.48 & 0.266 & 0.89 \\
PSZ2 G099.55+34.23 & 13.48 & 5.97 & 93.17 & 19.09 & 3.14e+25 & 6.44e+24 & 0.56 & 0.07 & 851.0 & 112.6 & circle & 5.95 & 0.237 & 0.84 \\
PSZ2 G116.50-44.47 & 12.62 & 6.73 & 23.23 & 8.29 & 1.42e+25 & 5.05e+24 & 3.94 & 0.78 & 187.8 & 36.0 & circle & 5.11 & 0.680 & 1.08 \\
PSZ2 G118.34+68.79 & 7.31 & 2.48 & 25.05 & 4.47 & 5.33e+24 & 9.52e+23 & 0.80 & 0.09 & 321.5 & 32.4 & circle & 8.58 & 0.208 & 1.34 \\
PSZ2 G123.00-35.52 & 8.28 & 1.86 & 20.43 & 4.27 & 1.13e+25 & 2.35e+24 & 2.23 & 0.35 & 228.4 & 34.4 & circle & 5.93 & 0.578 & 1.08 \\
PSZ2 G133.59+50.68 & 10.19 & 1.45 & 18.96 & 3.35 & 2.37e+25 & 4.18e+24 & 1.20 & 0.15 & 362.8 & 43.6 & circle & 7.07 & 0.257 & 0.92 \\
PSZ2 G163.61+34.30 & 8.50 & 2.19 & 17.02 & 3.71 & 2.87e+25 & 6.25e+24 & 1.50 & 0.24 & 324.7 & 44.9 & circle & 6.21 & 0.379 & 0.79 \\

==> tables/table_cw_sample.tex <==
PSZ2 G023.17+86.71 &  & 1.23e-01 & 1.00e-02 & 2.17e-02 & 2.65e-03 & C+X \\
PSZ2 G031.93+78.71 &  & 2.14e-01 & 1.53e-03 & 2.83e-02 & 2.39e-04 & X \\
PSZ2 G033.81+77.18 &  & 4.26e-01 & 1.77e-03 & 8.67e-03 & 2.43e-03 & C+X \\
PSZ2 G040.58+77.12 &  & 2.27e-01 & 6.40e-03 & 6.11e-03 & 6.80e-04 & C+X \\
PSZ2 G045.87+57.70 &  & 2.54e-01 & 5.10e-03 & 2.18e-02 & 7.02e-04 & X \\
PSZ2 G046.88+56.48 &  & 8.24e-02 & 4.15e-03 & 2.34e-02 & 1.75e-03 & C+X \\
PSZ2 G048.10+57.16 &  & 8.80e-02 & 2.87e-03 & 5.91e-02 & 7.59e-03 & C+X \\
PSZ2 G048.75+53.18 &  & 3.40e-01 & 8.41e-03 & 6.49e-03 & 1.22e-03 & C \\
PSZ2 G049.18+65.05 &  & 2.87e-01 & 1.71e-02 & 7.97e-03 & 3.10e-03 & C \\
PSZ2 G049.32+44.37 &  & 1.84e-01 & 6.00e-03 & 1.09e-02 & 1.10e-03 & C+X \\
PSZ2 G050.46+67.54 &  & 3.61e-01 & 5.14e-03 & 1.86e-03 & 5.16e-04 & C \\
PSZ2 G053.53+59.52 &  & 1.39e-01 & 2.72e-03 & 1.32e-02 & 3.49e-03 & C+X \\
PSZ2 G054.99+53.41 &  & 1.44e-01 & 1.09e-02 & 1.65e-02 & 3.19e-03 & C+X \\
PSZ2 G055.59+31.85 &  & 3.00e-01 & 1.49e-02 & 5.65e-03 & 3.84e-03 & C+X \\
PSZ2 G056.77+36.32 &  & 3.03e-01 & 1.05e-02 & 3.88e-03 & 1.78e-03 & C+X \\
PSZ2 G057.61+34.93 &  & 1.08e-01 & 4.11e-03 & 1.40e-02 & 1.02e-03 & C+X \\
PSZ2 G057.78+52.32 & E & 2.26e-01 & 1.83e-03 & 6.11e-03 & 4.55e-04 & X \\
PSZ2 G057.78+52.32 & W & 2.25e-01 & 5.74e-03 & 1.61e-02 & 1.44e-03 & X \\
PSZ2 G057.92+27.64 &  & 4.52e-01 & 1.96e-02 & 5.48e-03 & 3.93e-03 & C+X \\
PSZ2 G058.29+18.55 & E & 1.25e-01 & 1.53e-02 & 3.63e-02 & 2.22e-02 & C+X \\
PSZ2 G058.29+18.55 & W & 4.22e-01 & 3.26e-03 & 1.34e-02 & 5.43e-04 & X \\
PSZ2 G059.47+33.06 &  & 3.66e-01 & 3.98e-02 & 1.36e-02 & 9.59e-04 & C+X \\
PSZ2 G060.55+27.00 &  & 4.22e-01 & 1.05e-02 & 4.26e-03 & 8.72e-04 & C+X \\
PSZ2 G062.94+43.69 &  & 4.36e-01 & 3.40e-04 & 3.00e-03 & 1.95e-05 & X \\
PSZ2 G065.28+44.53 &  & 2.11e-01 & 6.56e-03 & 3.44e-02 & 1.78e-03 & C \\
PSZ2 G066.41+27.03 &  & 8.83e-02 & 8.98e-03 & 2.75e-02 & 2.28e-02 & C+X \\
PSZ2 G066.68+68.44 &  & 3.42e-01 & 8.91e-03 & 8.70e-03 & 3.25e-03 & C+X \\
PSZ2 G067.17+67.46 &  & 2.23e-01 & 8.98e-03 & 4.29e-02 & 1.61e-03 & C+X \\
PSZ2 G067.52+34.75 &  & 3.89e-01 & 2.42e-03 & 4.10e-03 & 2.71e-04 & X \\
PSZ2 G068.36+81.81 &  & 1.37e-01 & 3.05e-03 & 2.69e-02 & 8.34e-04 & X \\
PSZ2 G070.89+49.26 &  & 1.36e-01 & 4.25e-03 & 2.06e-02 & 1.20e-03 & X \\
PSZ2 G071.21+28.86 &  & 6.38e-02 & 4.45e-03 & 1.29e-02 & 2.08e-03 & X \\
PSZ2 G071.39+59.54 &  & 1.53e-01 & 1.51e-02 & 1.65e-02 & 3.03e-03 & C+X \\
PSZ2 G071.63+29.78 &  & 8.24e-02 & 3.34e-03 & 2.45e-02 & 1.38e-02 & C+X \\
PSZ2 G072.62+41.46 &  & 1.30e-01 & 7.29e-03 & 2.68e-02 & 5.08e-03 & C+X \\
PSZ2 G073.31+67.52 &  & 1.56e-01 & 1.42e-02 & 1.58e-02 & 2.81e-03 & C+X \\
PSZ2 G073.97-27.82 &  & 2.77e-01 & 5.97e-03 & 1.11e-02 & 5.59e-04 & C+X \\
PSZ2 G074.37+71.11 &  & 1.43e-01 & 2.00e-02 & 2.82e-02 & 6.10e-03 & C \\
PSZ2 G076.55+60.29 &  & 2.38e-01 & 1.70e-02 & 2.87e-02 & 3.84e-03 & C \\
PSZ2 G077.90-26.63 &  & 2.19e-01 & 7.61e-03 & 1.80e-02 & 1.05e-03 & C+X \\
PSZ2 G080.16+57.65 &  & 1.30e-01 & 1.12e-02 & 3.27e-02 & 2.05e-03 & C+X \\
PSZ2 G080.41-33.24 &  & 1.98e-01 & 1.72e-02 & 5.85e-02 & 1.31e-02 & C+X \\
PSZ2 G080.64+64.31 &  & 4.53e-01 & 1.24e-02 & 6.22e-03 & 1.50e-03 & C \\
PSZ2 G081.02+50.57 &  & 1.49e-01 & 5.22e-03 & 3.77e-02 & 1.37e-03 & X \\
PSZ2 G081.72+70.15 &  & 1.21e-01 & 1.80e-02 & 1.83e-02 & 5.38e-03 & C \\
PSZ2 G083.29-31.03 &  & 1.77e-01 & 1.27e-02 & 2.97e-02 & 1.07e-02 & C+X \\
PSZ2 G083.86+85.09 &  & 1.89e-01 & 9.11e-03 & 3.33e-02 & 4.09e-03 & C+X \\
PSZ2 G084.10+58.72 &  & 1.77e-01 & 2.79e-02 & 2.04e-02 & 9.05e-03 & C+X \\
PSZ2 G084.13-35.41 &  & 9.53e-02 & 5.82e-03 & 3.79e-02 & 2.14e-03 & X \\
PSZ2 G084.69+42.28 &  & 2.70e-01 & 4.30e-03 & 1.29e-02 & 5.93e-04 & X \\
PSZ2 G086.54-26.67 &  & 3.04e-01 & 6.40e-03 & 5.42e-03 & 8.78e-04 & C \\
PSZ2 G086.93+53.18 &  & 1.26e-01 & 1.86e-02 & 1.86e-02 & 3.51e-03 & C+X \\
PSZ2 G087.39+50.92 &  & 2.13e-01 & 1.16e-02 & 2.34e-02 & 2.13e-03 & X \\
PSZ2 G088.98+55.07 &  & 2.94e-01 & 1.20e-01 & 6.44e-02 & 1.62e-02 & C+X \\
PSZ2 G089.52+62.34 &  & 1.13e-01 & 9.41e-03 & 3.20e-02 & 2.26e-03 & C \\
PSZ2 G091.79-27.00 &  & 7.29e-02 & 6.16e-03 & 4.54e-02 & 2.52e-03 & X \\
PSZ2 G092.69+59.92 &  & 1.29e-01 & 4.45e-02 & 6.63e-02 & 4.53e-02 & C+X \\
PSZ2 G092.71+73.46 &  & 1.54e-01 & 5.69e-03 & 1.44e-02 & 2.21e-03 & C+X \\
PSZ2 G093.94-38.82 & EN & 2.14e-01 & 2.36e-03 & 4.07e-02 & 5.69e-04 & X \\
PSZ2 G093.94-38.82 & ES & 1.93e-01 & 2.30e-03 & 3.18e-02 & 5.75e-04 & X \\
PSZ2 G093.94-38.82 & W & 3.29e-01 & 3.09e-03 & 1.68e-02 & 5.35e-04 & X \\
PSZ2 G094.44+36.13 &  & 2.83e-01 & 2.85e-02 & 1.33e-02 & 4.92e-03 & C+X \\
PSZ2 G094.56+51.03 &  & 1.02e-01 & 4.14e-03 & 5.69e-02 & 1.67e-03 & X \\
PSZ2 G094.61-41.24 &  & 3.23e-01 & 1.26e-03 & 7.82e-03 & 2.16e-04 & X \\
PSZ2 G095.22+67.41 &  & 1.25e-01 & 2.28e-03 & 2.06e-02 & 8.51e-04 & X \\
PSZ2 G096.83+52.49 &  & 2.09e-01 & 3.63e-03 & 8.69e-03 & 8.71e-04 & C \\
PSZ2 G097.52+51.70 &  & 2.17e-01 & 8.06e-03 & 1.92e-02 & 1.10e-03 & X \\
PSZ2 G097.72+38.12 &  & 1.70e-01 & 6.56e-03 & 3.21e-02 & 7.91e-03 & C+X \\
PSZ2 G099.48+55.60 &  & 8.41e-02 & 4.91e-03 & 2.55e-02 & 3.21e-03 & C+X \\
PSZ2 G099.86+58.45 &  & 1.33e-01 & 1.04e-02 & 2.15e-02 & 5.58e-03 & C+X \\
PSZ2 G100.14+41.67 &  & 2.50e-01 & 3.02e-03 & 5.67e-02 & 5.84e-04 & C \\
PSZ2 G100.45-38.42 &  & 4.11e-01 & 1.50e-03 & 2.64e-03 & 1.35e-04 & X \\
PSZ2 G103.40-32.99 &  & 1.08e-01 & 1.21e-03 & 5.21e-03 & 5.06e-04 & X \\
PSZ2 G105.55+77.21 &  & 1.82e-01 & 2.31e-03 & 2.52e-02 & 6.40e-04 & X \\
PSZ2 G106.41+50.82 &  & 3.49e-01 & 2.12e-02 & 1.90e-02 & 1.22e-03 & C+X \\
PSZ2 G106.61+66.71 &  & 1.40e-01 & 3.20e-02 & 5.08e-02 & 7.99e-03 & C \\
PSZ2 G107.10+65.32 & N & 1.07e-01 & 5.96e-03 & 8.61e-02 & 1.15e-03 & C+X \\
PSZ2 G107.10+65.32 & S & 1.42e-01 & 6.93e-03 & 3.60e-02 & 2.18e-03 & C+X \\
PSZ2 G109.97+52.84 &  & 3.34e-01 & 5.04e-03 & 8.21e-03 & 8.83e-04 & C \\
PSZ2 G111.75+70.37 &  & 9.16e-02 & 6.56e-03 & 5.71e-02 & 3.19e-03 & C+X \\
PSZ2 G112.35-32.86 &  & 2.63e-01 & 9.71e-03 & 1.35e-02 & 1.41e-03 & X \\
PSZ2 G112.48+56.99 &  & 1.74e-01 & 4.69e-03 & 4.60e-03 & 9.61e-04 & C \\
PSZ2 G113.29-29.69 &  & 1.69e-01 & 1.02e-02 & 1.33e-02 & 5.02e-03 & C+X \\
PSZ2 G113.91-37.01 &  & 1.57e-01 & 1.65e-02 & 4.60e-02 & 2.54e-03 & C+X \\
PSZ2 G114.31+64.89 &  & 1.66e-01 & 2.70e-02 & 1.28e-02 & 1.92e-03 & C+X \\
PSZ2 G114.79-33.71 &  & 1.53e-01 & 9.18e-03 & 7.39e-03 & 4.54e-03 & C+X \\
PSZ2 G114.99+70.36 &  & 1.46e-01 & 5.90e-03 & 1.72e-02 & 1.80e-03 & C \\
PSZ2 G116.32-36.33 & N & 1.50e-01 & 1.70e-02 & 1.24e-02 & 4.73e-03 & C+X \\
PSZ2 G116.32-36.33 & S & 2.97e-01 & 1.26e-02 & 9.13e-03 & 1.50e-03 & X \\
PSZ2 G116.50-44.47 &  & 1.30e-01 & 6.75e-03 & 5.60e-02 & 2.37e-03 & X \\
PSZ2 G121.03+57.02 &  & 9.77e-02 & 7.83e-03 & 1.10e-01 & 3.74e-03 & C \\
PSZ2 G121.13+49.64 &  & 9.88e-02 & 5.27e-03 & 3.28e-02 & 1.94e-03 & X \\
PSZ2 G123.00-35.52 &  & 1.56e-01 & 5.28e-03 & 2.39e-02 & 1.08e-03 & X \\
PSZ2 G123.66+67.25 &  & 2.50e-01 & 3.05e-02 & 1.59e-02 & 5.27e-03 & C \\
PSZ2 G124.20-36.48 & N & 3.06e-01 & 3.56e-03 & 5.41e-02 & 8.91e-04 & C+X \\
PSZ2 G124.20-36.48 & S & 1.01e-01 & 1.04e-02 & 1.90e-02 & 6.16e-03 & C+X \\
PSZ2 G125.71+53.86 &  & 1.96e-01 & 1.68e-02 & 1.04e-02 & 3.56e-03 & C+X \\
PSZ2 G126.61-37.63 &  & 1.70e-01 & 5.69e-03 & 8.77e-03 & 1.09e-03 & X \\
PSZ2 G127.50-30.52 &  & 1.16e-01 & 7.32e-03 & 1.39e-02 & 2.04e-03 & X \\
PSZ2 G132.54-42.16 &  & 2.11e-01 & 8.94e-03 & 2.55e-03 & 1.58e-03 & X \\
PSZ2 G133.59+50.68 &  & 9.27e-02 & 5.08e-03 & 1.94e-02 & 2.18e-03 & X \\
PSZ2 G133.60+69.04 &  & 8.67e-02 & 8.92e-03 & 3.80e-02 & 3.49e-03 & C \\
PSZ2 G134.70+48.91 &  & 2.52e-01 & 2.79e-02 & 5.34e-03 & 1.98e-03 & C+X \\
PSZ2 G135.17+65.43 &  & 1.05e-01 & 1.87e-02 & 4.72e-02 & 7.64e-03 & C \\
PSZ2 G135.19+57.88 &  & 1.66e-01 & 9.31e-03 & 1.33e-02 & 2.56e-03 & C \\
PSZ2 G136.92+59.46 &  & 9.37e-02 & 2.33e-03 & 8.87e-02 & 1.22e-03 & X \\
PSZ2 G137.74-27.08 &  & 1.46e-01 & 2.35e-03 & 4.31e-02 & 6.91e-04 & X \\
PSZ2 G138.32-39.82 &  & 1.98e-01 & 6.58e-03 & 1.32e-02 & 1.33e-03 & C \\
PSZ2 G139.18+56.37 &  & 8.60e-02 & 5.90e-03 & 4.70e-02 & 8.49e-03 & C+X \\
PSZ2 G143.26+65.24 &  & 1.42e-01 & 2.62e-02 & 2.46e-02 & 1.49e-03 & C+X \\
PSZ2 G145.65+59.30 &  & 1.44e-01 & 6.56e-03 & 1.20e-02 & 1.45e-03 & X \\
PSZ2 G148.36+75.23 &  & 2.06e-01 & 9.02e-03 & 5.27e-02 & 2.43e-03 & C \\
PSZ2 G149.22+54.18 &  & 1.36e-01 & 3.42e-03 & 3.72e-03 & 8.17e-04 & C \\
PSZ2 G149.75+34.68 &  & 1.72e-01 & 3.39e-03 & 6.13e-02 & 3.66e-03 & C+X \\
PSZ2 G150.56+58.32 &  & 1.33e-01 & 1.62e-02 & 3.16e-02 & 1.77e-02 & C+X \\
PSZ2 G151.19+48.27 &  & 7.73e-02 & 8.77e-03 & 2.41e-02 & 1.18e-02 & C+X \\
PSZ2 G160.83+81.66 &  & 2.78e-01 & 3.08e-02 & 1.72e-02 & 3.92e-03 & C+X \\
PSZ2 G163.69+53.52 &  & 1.98e-01 & 5.88e-03 & 8.31e-03 & 1.41e-03 & C \\
PSZ2 G163.87+48.54 &  & 4.61e-01 & 3.51e-03 & 1.61e-03 & 3.40e-04 & C \\
PSZ2 G164.65+46.37 &  & 2.46e-01 & 1.00e-02 & 6.05e-02 & 2.10e-03 & C \\
PSZ2 G165.06+54.13 &  & 1.88e-01 & 5.22e-03 & 1.77e-02 & 1.53e-03 & C \\
PSZ2 G165.46+66.15 &  & 6.96e-02 & 5.22e-03 & 3.31e-02 & 3.13e-03 & C \\
PSZ2 G166.09+43.38 &  & 1.84e-01 & 6.80e-03 & 1.83e-02 & 5.71e-03 & C+X \\
PSZ2 G166.62+42.13 &  & 6.85e-02 & 5.52e-03 & 3.48e-02 & 3.03e-03 & C \\
PSZ2 G168.33+69.73 &  & 2.64e-01 & 3.00e-02 & 1.91e-02 & 4.29e-03 & C \\
PSZ2 G170.98+39.45 &  & 1.14e-01 & 1.61e-02 & 2.69e-02 & 6.51e-03 & C \\
PSZ2 G172.63+35.15 &  & 1.84e-01 & 8.75e-03 & 2.01e-02 & 2.14e-03 & C \\
PSZ2 G172.74+65.30 &  & 2.18e-01 & 1.10e-02 & 2.44e-02 & 1.69e-02 & C+X \\
PSZ2 G175.60+35.47 &  & 2.66e-01 & 1.13e-02 & 1.05e-02 & 2.00e-03 & C \\
PSZ2 G176.27+37.54 &  & 2.43e-01 & 1.69e-02 & 1.90e-02 & 3.87e-03 & C \\
PSZ2 G179.09+60.12 &  & 5.15e-01 & 6.11e-03 & 6.54e-03 & 2.17e-03 & C+X \\
PSZ2 G180.60+76.65 &  & 2.89e-01 & 6.39e-03 & 2.41e-03 & 5.32e-04 & C \\
PSZ2 G180.88+31.04 &  & 1.01e-01 & 1.15e-02 & 1.83e-02 & 4.22e-03 & X \\
PSZ2 G181.06+48.47 &  & 1.41e-01 & 1.05e-02 & 6.95e-02 & 3.04e-03 & C \\
PSZ2 G182.59+55.83 &  & 2.86e-01 & 1.26e-02 & 5.95e-03 & 9.26e-04 & C+X \\
PSZ2 G183.90+42.99 &  & 1.56e-01 & 4.77e-03 & 1.82e-02 & 1.13e-03 & X \\
PSZ2 G184.68+28.91 &  & 2.93e-01 & 1.47e-02 & 7.89e-03 & 2.99e-03 & C+X \\
PSZ2 G186.37+37.26 &  & 1.47e-01 & 8.43e-03 & 9.89e-03 & 5.32e-03 & C+X \\
PSZ2 G186.99+38.65 &  & 1.99e-01 & 8.38e-03 & 3.85e-02 & 2.11e-03 & C \\
PSZ2 G187.53+21.92 &  & 3.04e-01 & 1.59e-02 & 7.20e-03 & 5.27e-03 & C+X \\
PSZ2 G189.31+59.24 &  & 2.45e-01 & 3.64e-03 & 4.76e-02 & 7.56e-04 & C \\
PSZ2 G190.61+66.46 &  & 1.05e-01 & 1.61e-02 & 2.87e-02 & 5.77e-03 & C \\
PSZ2 G192.18+56.12 &  & 1.72e-01 & 7.12e-03 & 1.70e-02 & 1.12e-02 & C+X \\
PSZ2 G193.63+54.85 &  & 1.67e-01 & 7.38e-03 & 5.62e-02 & 1.86e-03 & X \\
PSZ2 G194.98+54.12 &  & 1.84e-01 & 1.37e-02 & 6.07e-02 & 3.54e-03 & C \\
PSZ2 G195.60+44.06 & E1 & 9.39e-02 & 5.86e-03 & 1.94e-02 & 2.35e-03 & X \\
PSZ2 G195.60+44.06 & E2 & 1.23e-01 & 7.51e-03 & 4.63e-02 & 1.97e-02 & C+X \\
PSZ2 G195.60+44.06 & W1 & 2.83e-01 & 7.56e-03 & 8.57e-03 & 9.76e-04 & X \\
PSZ2 G195.60+44.06 & W2 & 9.70e-02 & 2.07e-03 & 4.79e-02 & 7.30e-04 & X \\
PSZ2 G205.90+73.76 &  & 2.12e-01 & 1.79e-02 & 1.35e-02 & 3.23e-03 & C \\

==> tables/table_full_sample.tex <==
PSZ2 G023.17+86.71 & 196.4731 & 26.5262 & 0.306 & 5.03 & 0.56 & 1093 & 41 & 1 & 0.093 & RH & C/X & New RH \\
PSZ2 G031.93+78.71 & 205.4709 & 26.3684 & 0.072 & 2.72 & 0.24 & 966 & 28 & 2 & 0.099 & RH, U & C/X & U emission on the SE, outside R500 \\
PSZ2 G033.81+77.18 & 207.2221 & 26.5946 & 0.062 & 4.47 & 0.14 & 1144 & 12 & 3 & 0.102 & N/A & C/X & --- \\
PSZ2 G040.58+77.12 & 207.3622 & 28.0946 & 0.075 & 2.63 & 0.22 & 955 & 26 & 2 & 0.112 & RH & C/X & New RH \\
PSZ2 G045.13+67.78 & 217.9958 & 29.5567 & 0.219 & 4.83 & 0.45 & 1113 & 35 & 1 & 0.105 & NDE & --- & --- \\
PSZ2 G045.87+57.70 & 229.5874 & 29.4696 & 0.611 & 7.03 & 0.68 & 1085 & 35 & 1 & 0.110 & RH & X & --- \\
PSZ2 G046.88+56.48 & 231.0469 & 29.9129 & 0.115 & 5.31 & 0.23 & 1191 & 17 & 1 & 0.124 & RH & C/X & --- \\
PSZ2 G048.10+57.16 & 230.3161 & 30.6278 & 0.078 & 3.59 & 0.21 & 1058 & 21 & 1 & 0.101 & RH, RR & C/X & --- \\
PSZ2 G048.75+53.18 & 234.9669 & 30.6960 & 0.098 & 2.53 & 0.31 & 935 & 39 & 1 & 0.124 & NDE & C & --- \\
PSZ2 G049.18+65.05 & 221.1194 & 31.2334 & 0.234 & 4.73 & 0.49 & 1099 & 38 & 1 & 0.096 & NDE & C & --- \\
PSZ2 G049.32+44.37 & 245.1404 & 29.8941 & 0.097 & 3.67 & 0.26 & 1059 & 25 & 2 & 0.116 & RH & C/X & New RH \\
PSZ2 G050.46+67.54 & 218.1680 & 31.5879 & 0.131 & 2.92 & 0.34 & 971 & 38 & 1 & 0.098 & NDE & C & --- \\
PSZ2 G052.08+46.13 & 243.4439 & 32.0814 &  &  &  &  &  & 1 & 0.093 & NDE & --- & --- \\
PSZ2 G053.53+59.52 & 227.5546 & 33.4915 & 0.113 & 5.85 & 0.23 & 1231 & 16 & 1 & 0.093 & RH, U & C/X & U emissions in the outskirts \\
PSZ2 G053.80+36.49 & 254.9008 & 31.7432 &  &  &  &  &  & 1 & 0.115 & NDE & --- & --- \\
PSZ2 G054.85+54.30 & 233.8283 & 34.3446 & 0.235 & 4.39 & 0.46 & 1072 & 38 & 2 & 0.099 & NDE & --- & --- \\
PSZ2 G054.99+53.41 & 234.9018 & 34.4313 & 0.229 & 5.73 & 0.38 & 1174 & 26 & 3 & 0.122 & N/A & C/X & --- \\
PSZ2 G055.59+31.85 & 260.6150 & 32.1354 & 0.224 & 7.78 & 0.31 & 1302 & 17 & 1 & 0.106 & RH & C/X & --- \\
PSZ2 G055.80+32.90 & 259.4624 & 32.5608 & 0.105 & 2.58 & 0.31 & 939 & 37 & 1 & 0.124 & NDE & --- & --- \\
PSZ2 G056.14+28.06 & 265.0748 & 31.6030 & 0.426 & 5.53 & 0.57 & 1077 & 37 & 1 & 0.133 & NDE & --- & --- \\
PSZ2 G056.38+23.36 & 270.3845 & 30.3962 &  &  &  &  &  & 2 & 0.226 & NDE & --- & --- \\
PSZ2 G056.62+88.42 & 194.4923 & 27.7528 & 0.045 & 3.30 & 0.07 & 1039 & 7 & -1 & -1.000 & --- & --- & Toward the direction of the Coma cluster \\
PSZ2 G056.77+36.32 & 255.6663 & 34.0511 & 0.095 & 4.38 & 0.20 & 1124 & 17 & 1 & 0.123 & RH & C/X & New RH \\
PSZ2 G057.61+34.93 & 257.4672 & 34.4613 & 0.080 & 3.73 & 0.19 & 1071 & 18 & 2 & 0.140 & RR, U & C/X & U emission in the center \\
PSZ2 G057.73+51.58 & 237.1413 & 36.1034 & 0.238 & 5.59 & 0.51 & 1160 & 36 & 1 & 0.113 & NDE & --- & --- \\
PSZ2 G057.78+52.32 & 236.2149 & 36.1219 & 0.065 & 2.38 & 0.22 & 926 & 28 & 1 & 0.124 & NDE & C/X & --- \\
PSZ2 G057.80+88.00 & 194.9118 & 27.9537 & 0.023 & 7.17 & 0.09 & 1356 & 6 & -1 & -1.000 & --- & --- & Coma cluster \\
PSZ2 G057.92+27.64 & 266.0678 & 32.9986 & 0.076 & 2.68 & 0.21 & 961 & 25 & 2 & 0.118 & NDE & C/X & --- \\
PSZ2 G058.29+18.55 & 276.3360 & 30.4320 & 0.065 & 3.88 & 0.17 & 1091 & 16 & 3 & 0.555 & N/A & C/X & --- \\
PSZ2 G058.31+41.96 & 249.0508 & 36.0554 &  &  &  &  &  & 1 & 0.095 & NDE & --- & --- \\
PSZ2 G059.18+32.91 & 260.2029 & 35.3248 & 0.383 & 5.21 & 0.56 & 1074 & 39 & 1 & 0.145 & NDE & --- & --- \\
PSZ2 G059.29+44.49 & 245.9901 & 36.9729 & 0.343 & 5.76 & 0.69 & 1128 & 45 & 1 & 0.123 & NDE & --- & --- \\
PSZ2 G059.47+33.06 & 260.0786 & 35.6002 & 0.387 & 6.09 & 0.58 & 1129 & 36 & 2 & 0.170 & U & C/X & --- \\
PSZ2 G059.52+16.23 & 279.3393 & 30.6642 & 0.284 & 4.37 & 0.55 & 1052 & 45 & 3 & 2.503 & N/A & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G059.76+14.59 & 281.1949 & 30.2468 & 0.303 & 4.80 & 0.51 & 1077 & 38 & 3 & 0.457 & N/A & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G060.10+15.59 & 280.2784 & 30.9322 & 0.190 & 4.67 & 0.47 & 1112 & 37 & -1 & -1.000 & --- & --- & --- \\
PSZ2 G060.16+64.50 & 221.0737 & 35.9376 & 0.361 & 5.00 & 0.63 & 1068 & 45 & 1 & 0.088 & NDE & --- & --- \\
PSZ2 G060.55+27.00 & 267.5745 & 35.0761 & 0.171 & 3.48 & 0.41 & 1015 & 40 & 2 & 0.147 & NDE & C/X & --- \\
PSZ2 G061.75+88.11 & 194.7270 & 28.0231 & 0.044 & 3.40 & 0.63 & 1051 & 66 & -1 & -1.000 & --- & --- & Toward the direction of the Coma cluster \\
PSZ2 G062.94+43.69 & 247.1565 & 39.5602 & 0.030 & 2.87 & 0.12 & 997 & 14 & 3 & 0.123 & N/A & C/X & --- \\
PSZ2 G063.38+53.44 & 234.5073 & 39.4147 & 0.422 & 6.24 & 0.60 & 1123 & 36 & 1 & 0.111 & cRH & --- & New cRH \\
PSZ2 G065.28+44.53 & 246.0751 & 41.2470 & 0.182 & 3.90 & 0.48 & 1050 & 44 & 1 & 0.099 & NDE & C & --- \\
PSZ2 G065.45+78.10 & 204.8180 & 33.0102 & 0.273 & 4.07 & 0.53 & 1031 & 46 & 1 & 0.111 & NDE & --- & --- \\
PSZ2 G065.79+41.80 & 249.7168 & 41.5990 & 0.336 & 5.22 & 0.59 & 1094 & 42 & 1 & 0.094 & NDE & --- & --- \\
PSZ2 G065.89+31.59 & 263.2231 & 40.6419 & 0.133 & 2.74 & 0.36 & 949 & 42 & 1 & 0.119 & NDE & --- & --- \\
PSZ2 G066.26+20.82 & 276.8511 & 38.2587 & 0.278 & 4.13 & 0.50 & 1034 & 42 & 2 & 0.194 & NDE & --- & --- \\
PSZ2 G066.34+26.14 & 270.3078 & 39.8546 & 0.622 & 6.10 & 0.67 & 1031 & 38 & 2 & 0.110 & cRH & --- & New cRH. Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G066.41+27.03 & 269.2019 & 40.1327 & 0.576 & 7.70 & 0.53 & 1134 & 26 & 1 & 0.118 & RH & C/X & New RH \\
PSZ2 G066.68+68.44 & 215.4320 & 37.2821 & 0.163 & 3.79 & 0.34 & 1047 & 32 & 1 & 0.083 & NDE & C/X & --- \\
PSZ2 G066.85+22.48 & 275.0416 & 39.2985 & 0.190 & 3.14 & 0.41 & 974 & 43 & 3 & 0.354 & N/A & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G067.17+67.46 & 216.5032 & 37.8160 & 0.171 & 7.24 & 0.26 & 1295 & 16 & 2 & 0.192 & U & C/X & --- \\
PSZ2 G067.52+34.75 & 259.3134 & 42.4618 & 0.175 & 4.54 & 0.34 & 1107 & 28 & 2 & 0.112 & NDE & C/X & --- \\
PSZ2 G068.36+81.81 & 200.6946 & 31.6565 & 0.308 & 6.60 & 0.43 & 1195 & 26 & 2 & 0.163 & NDE & X & --- \\
PSZ2 G069.39+68.05 & 215.4044 & 38.3613 & 0.762 & 5.69 & 0.77 & 952 & 43 & 2 & 0.183 & cRH, cRR & --- & New cRH and cRR. Redshift updated from Buddendiek et al. (2015) \\
PSZ2 G070.89+49.26 & 239.1791 & 44.6533 & 0.610 & 6.46 & 0.69 & 1055 & 38 & 1 & 0.087 & NDE & X & --- \\
PSZ2 G071.21+28.86 & 268.0130 & 44.6695 & 0.366 & 6.75 & 0.45 & 1178 & 26 & 1 & 0.101 & RH, RR & X & Double RR \\
PSZ2 G071.39+59.54 & 225.3359 & 42.3464 & 0.292 & 5.87 & 0.42 & 1157 & 27 & 2 & 0.084 & RH* & C/X & New RH* \\
PSZ2 G071.63+29.78 & 266.8257 & 45.1899 & 0.157 & 4.13 & 0.29 & 1080 & 25 & 1 & 0.101 & NDE & C/X & Possible revived fossil plasma in the S \\
PSZ2 G072.62+41.46 & 250.0941 & 46.7103 & 0.228 & 11.69 & 0.26 & 1490 & 11 & 3 & 0.111 & N/A & C/X & --- \\
PSZ2 G073.31+67.52 & 215.1737 & 39.9245 & 0.609 & 6.74 & 0.59 & 1071 & 31 & 3 & 0.475 & N/A & C/X & --- \\
PSZ2 G073.97-27.82 & 328.4233 & 17.6986 & 0.233 & 9.80 & 0.28 & 1402 & 13 & 2 & 0.216 & NDE & C/X & --- \\
PSZ2 G074.37+71.11 & 210.9114 & 38.4697 & 0.485 & 5.75 & 0.58 & 1067 & 36 & 3 & 0.169 & N/A & C & --- \\
PSZ2 G075.08+19.83 & 281.6991 & 45.7759 & 0.200 & 3.45 & 0.38 & 1002 & 37 & -1 & -1.000 & --- & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G076.55+60.29 & 223.0302 & 44.4554 & 0.287 & 4.13 & 0.48 & 1031 & 40 & 1 & 0.067 & RH* & C & New RH*. Redshift updated from Streblyanska et al. (2018) \\
PSZ2 G077.90-26.63 & 330.2281 & 20.9701 & 0.147 & 5.06 & 0.26 & 1160 & 20 & 2 & 0.216 & RH* & C/X & New RH* \\
PSZ2 G080.16+57.65 & 225.2369 & 47.2874 & 0.088 & 2.51 & 0.21 & 937 & 26 & 1 & 0.127 & RR & C/X & --- \\
PSZ2 G080.41-33.24 & 336.5396 & 17.3767 & 0.107 & 3.77 & 0.27 & 1066 & 26 & 1 & 0.139 & NDE & C/X & Revived fossil plasma \\
PSZ2 G080.55-24.82 & 330.8550 & 23.9105 & 0.266 & 4.28 & 0.53 & 1051 & 43 & 1 & 0.135 & NDE & --- & --- \\
PSZ2 G080.64+64.31 & 216.8313 & 44.1308 & 0.502 & 5.23 & 0.59 & 1026 & 39 & 1 & 0.133 & NDE & C & --- \\
PSZ2 G080.70+48.31 & 238.2988 & 51.1483 & 0.235 & 3.20 & 0.41 & 965 & 41 & 1 & 0.068 & cRH & --- & New cRH \\
PSZ2 G081.02+50.57 & 234.8082 & 50.6137 & 0.501 & 4.69 & 0.54 & 991 & 38 & 1 & 0.061 & RH & X & New RH \\
PSZ2 G081.72+70.15 & 210.0995 & 41.0129 & 0.250 & 4.16 & 0.44 & 1047 & 37 & 1 & 0.097 & U & C & Two uncertain sources located to the W with respect to the bulk of the X-ray emission \\
PSZ2 G083.14+66.57 & 213.4445 & 43.6523 & 0.089 & 2.07 & 0.26 & 878 & 36 & 2 & 0.077 & NDE & --- & --- \\
PSZ2 G083.29-31.03 & 337.1296 & 20.6221 & 0.412 & 8.27 & 0.44 & 1239 & 22 & 1 & 0.118 & RH & C/X & New RH \\
PSZ2 G083.86+85.09 & 196.4623 & 30.8931 & 0.183 & 4.66 & 0.33 & 1114 & 27 & 1 & 0.079 & NDE & C/X & --- \\
PSZ2 G084.10+58.72 & 222.3158 & 48.5589 & 0.731 & 5.40 & 0.62 & 947 & 36 & 1 & 0.073 & RH & C/X & --- \\
PSZ2 G084.13-35.41 & 340.4853 & 17.5233 & 0.314 & 5.50 & 0.58 & 1122 & 40 & 2 & 0.127 & RH, U & X & New RH. U emission to the S of the RH \\
PSZ2 G084.69+42.28 & 246.7659 & 55.4802 & 0.130 & 2.70 & 0.26 & 946 & 31 & 1 & 0.068 & NDE & X & --- \\
PSZ2 G085.23+39.42 & 251.6292 & 56.4674 & 0.257 & 3.88 & 0.39 & 1021 & 35 & 1 & 0.083 & cRH & --- & New cRH \\
PSZ2 G086.28+74.76 & 204.4773 & 38.8708 & 0.699 & 5.61 & 0.71 & 972 & 41 & 3 & 0.091 & N/A & --- & Redshift updated from Streblyanska et al. (2018) \\
PSZ2 G086.43-24.95 & 335.5578 & 27.1430 & 0.231 & 3.81 & 0.50 & 1024 & 46 & 1 & 0.127 & NDE & --- & --- \\
PSZ2 G086.54-26.67 & 336.7802 & 25.8145 & 0.165 & 3.45 & 0.39 & 1015 & 39 & 1 & 0.120 & NDE & C & --- \\
PSZ2 G086.58+73.11 & 205.8750 & 40.1328 & 0.222 & 3.83 & 0.50 & 1029 & 45 & 1 & 0.073 & cRR, U & --- & New cRR. U emission in the center \\
PSZ2 G086.93+53.18 & 228.4787 & 52.7984 & 0.675 & 5.45 & 0.51 & 971 & 30 & 1 & 0.101 & RH & C/X & --- \\
PSZ2 G087.39-34.58 & 342.3068 & 19.7139 & 0.760 & 6.06 & 0.63 & 973 & 34 & 2 & 0.184 & NDE & --- & Redshift updated from Streblyanska et al. (2018) \\
PSZ2 G087.39+50.92 & 231.5690 & 54.1431 & 0.748 & 5.16 & 0.57 & 927 & 34 & 3 & 0.098 & N/A & X & --- \\
PSZ2 G087.44-21.56 & 334.0988 & 30.4251 & 0.258 & 4.15 & 0.51 & 1043 & 43 & 1 & 0.120 & NDE & --- & --- \\
PSZ2 G088.53+41.18 & 247.3887 & 58.5338 & 0.133 & 2.56 & 0.34 & 929 & 42 & 1 & 0.076 & NDE & --- & Complex radio emission associated to the brightest optical galaxy \\
PSZ2 G088.98+55.07 & 224.7806 & 52.8020 & 0.702 & 4.92 & 0.62 & 929 & 39 & 3 & 0.105 & N/A & C/X & --- \\
PSZ2 G089.39+69.36 & 208.4259 & 43.4835 & 0.680 & 5.75 & 0.72 & 987 & 41 & 1 & 0.067 & cRH & --- & --- \\
PSZ2 G089.52+62.34 & 215.5299 & 48.4769 & 0.070 & 1.83 & 0.19 & 847 & 30 & 2 & 0.078 & RR & C & Two RR located in the N \\
PSZ2 G091.27-38.62 & 347.3346 & 17.8953 & 0.105 & 3.14 & 0.39 & 1003 & 42 & 2 & 0.146 & NDE & --- & Redshift updated from Barrena et al. (2018) \\
PSZ2 G091.79-27.00 & 341.3603 & 28.1444 & 0.362 & 6.31 & 0.48 & 1154 & 29 & 1 & 0.104 & RR & X & New RR \\
PSZ2 G092.11-33.73 & 345.4059 & 22.4833 &  &  &  &  &  & 2 & 0.161 & NDE & --- & --- \\
PSZ2 G092.46-35.22 & 346.4589 & 21.3244 &  &  &  &  &  & 1 & 0.141 & NDE & --- & --- \\
PSZ2 G092.69+59.92 & 216.6347 & 51.2521 & 0.462 & 4.79 & 0.60 & 1013 & 43 & 1 & 0.078 & NDE & C/X & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G092.71+73.46 & 203.8014 & 41.0004 & 0.228 & 8.13 & 0.27 & 1320 & 14 & 3 & 0.075 & N/A & C/X & --- \\
PSZ2 G093.04-32.38 & 345.4276 & 24.0403 & 0.512 & 6.34 & 0.72 & 1090 & 42 & 2 & 0.200 & NDE & --- & Redshift updated from Barrena et al. (2018) \\
PSZ2 G093.71-30.90 & 345.1839 & 25.6114 &  &  &  &  &  & 3 & 0.350 & N/A & --- & --- \\
PSZ2 G093.94-38.82 & 349.3656 & 18.7010 & 0.042 & 2.22 & 0.17 & 912 & 23 & 1 & 0.192 & U & C/X & --- \\
PSZ2 G094.44+36.13 & 255.2898 & 64.2391 & 0.453 & 4.09 & 0.43 & 964 & 34 & 1 & 0.078 & NDE & C/X & --- \\
PSZ2 G094.56+51.03 & 227.0614 & 57.8918 & 0.539 & 5.87 & 0.44 & 1051 & 26 & 3 & 0.086 & N/A & X & --- \\
PSZ2 G094.61-41.24 & 350.9896 & 16.7655 & 0.042 & 1.76 & 0.23 & 845 & 37 & 2 & 0.128 & U & C/X & --- \\
PSZ2 G095.00-37.14 & 349.3564 & 20.5736 &  &  &  &  &  & 1 & 0.144 & NDE & --- & --- \\
PSZ2 G095.22+67.41 & 207.8526 & 46.3557 & 0.062 & 1.50 & 0.21 & 795 & 38 & 1 & 0.084 & U & X & --- \\
PSZ2 G095.29+44.13 & 238.1346 & 62.0545 & 0.331 & 4.03 & 0.35 & 1006 & 29 & 2 & 0.103 & cRH* & --- & New cRH* \\
PSZ2 G096.14+56.24 & 218.8388 & 55.1414 & 0.140 & 2.77 & 0.25 & 951 & 28 & 2 & 0.086 & NDE & --- & --- \\
PSZ2 G096.43-20.89 & 342.0362 & 35.5560 & 0.350 & 5.39 & 0.51 & 1100 & 34 & 2 & 0.122 & cRR & --- & New cRR. Redshift updated from Boada et al. (2019) \\
PSZ2 G096.83+52.49 & 223.2488 & 58.0366 & 0.318 & 4.92 & 0.37 & 1080 & 27 & 1 & 0.073 & RH & C & --- \\
PSZ2 G097.15+39.20 & 246.9034 & 65.3963 & 0.206 & 2.94 & 0.32 & 948 & 34 & 1 & 0.088 & NDE & --- & --- \\
PSZ2 G097.52+51.70 & 223.8162 & 58.8752 & 0.700 & 5.18 & 0.51 & 946 & 31 & 2 & 0.105 & U & X & --- \\
PSZ2 G097.72+38.12 & 248.9776 & 66.2023 & 0.171 & 6.59 & 0.16 & 1255 & 10 & 1 & 0.076 & RH & C/X & --- \\
PSZ2 G097.78+46.95 & 231.0525 & 62.0227 & 0.338 & 3.43 & 0.39 & 950 & 36 & 2 & 0.104 & NDE & --- & --- \\
PSZ2 G098.30-41.15 & 353.5972 & 18.0003 & 0.436 & 7.05 & 0.61 & 1164 & 34 & 1 & 0.100 & cRH & --- & New cRH \\
PSZ2 G098.38+77.22 & 199.6059 & 38.5853 & 0.780 & 6.62 & 0.71 & 994 & 36 & 1 & 0.102 & NDE & --- & Redshift updated from Boada et al. (2019) \\
PSZ2 G098.39+57.68 & 215.5698 & 54.9011 &  &  &  &  &  & 1 & 0.091 & NDE & --- & --- \\
PSZ2 G098.44+56.59 & 216.7791 & 55.7497 & 0.132 & 2.83 & 0.27 & 960 & 30 & 1 & 0.090 & NDE & --- & --- \\
PSZ2 G098.62+51.76 & 222.8271 & 59.3306 & 0.298 & 3.35 & 0.48 & 958 & 47 & 2 & 0.075 & NDE & --- & Redshift updated from Streblyanska et al. (2018) \\
PSZ2 G098.75-28.63 & 348.4410 & 29.6117 &  &  &  &  &  & 2 & 0.113 & NDE & --- & --- \\
PSZ2 G099.24+42.54 & 238.0378 & 65.3405 & 0.223 & 2.80 & 0.39 & 927 & 43 & 1 & 0.104 & U & --- & U emissions in the center and outskirts \\
PSZ2 G099.48+37.72 & 248.6714 & 67.6423 & 0.167 & 2.51 & 0.28 & 911 & 34 & 1 & 0.104 & U & --- & --- \\
PSZ2 G099.48+55.60 & 217.1485 & 56.8766 & 0.105 & 2.81 & 0.21 & 967 & 25 & 1 & 0.098 & RR & C/X & New RR. Double RR \\
PSZ2 G099.55+34.23 & 257.6109 & 68.7321 & 0.310 & 3.61 & 0.38 & 977 & 34 & 1 & 0.112 & cRH*, U & --- & New cRH*. U emission in the W. Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G099.86+58.45 & 213.6782 & 54.7836 & 0.630 & 6.85 & 0.49 & 1067 & 25 & 2 & 0.075 & RH & C/X & --- \\
PSZ2 G100.14+41.67 & 239.0257 & 66.3545 & 0.234 & 4.04 & 0.28 & 1044 & 24 & 3 & 0.315 & N/A & C & --- \\
PSZ2 G100.22-29.64 & 350.2543 & 29.2136 & 0.485 & 7.64 & 0.59 & 1173 & 30 & 2 & 0.135 & NDE & --- & --- \\
PSZ2 G100.22+33.81 & 258.4193 & 69.3734 & 0.598 & 4.61 & 0.47 & 947 & 33 & 2 & 0.169 & NDE & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G100.45-38.42 & 354.1311 & 21.1519 & 0.057 & 1.84 & 0.27 & 853 & 42 & 1 & 0.143 & NDE & C/X & Revived fossil plasma \\
PSZ2 G100.96-24.07 & 348.3483 & 34.5796 & 0.424 & 5.70 & 0.73 & 1089 & 47 & 2 & 0.119 & cRH & --- & --- \\
PSZ2 G101.52-29.98 & 351.5963 & 29.3258 & 0.227 & 4.88 & 0.52 & 1114 & 39 & 1 & 0.114 & NDE & --- & --- \\
PSZ2 G102.90-31.04 & 353.3020 & 28.7678 & 0.592 & 6.73 & 0.72 & 1078 & 39 & 2 & 0.111 & NDE & --- & --- \\
PSZ2 G103.40-32.99 & 354.5043 & 27.0818 & 0.031 & 1.51 & 0.13 & 805 & 23 & 3 & 0.164 & N/A & X & --- \\
PSZ2 G104.15-38.85 & 357.2018 & 21.7235 &  &  &  &  &  & 1 & 0.095 & NDE & --- & --- \\
PSZ2 G105.55+77.21 & 197.7544 & 39.2463 & 0.072 & 2.20 & 0.22 & 900 & 30 & 1 & 0.140 & U & X & --- \\
PSZ2 G105.76+54.73 & 212.5897 & 59.6801 & 0.316 & 4.41 & 0.45 & 1042 & 36 & 1 & 0.149 & NDE & --- & --- \\
PSZ2 G105.82-38.36 & 358.3931 & 22.5789 &  &  &  &  &  & 1 & 0.098 & NDE & --- & --- \\
PSZ2 G106.41+50.82 & 216.3149 & 63.1860 & 0.139 & 2.89 & 0.25 & 964 & 27 & 1 & 0.073 & U & C/X & --- \\
PSZ2 G106.61+66.71 & 202.6355 & 49.1529 & 0.331 & 4.67 & 0.56 & 1056 & 42 & 1 & 0.055 & RH & C & --- \\
PSZ2 G107.10+65.32 & 203.1777 & 50.5183 & 0.280 & 8.22 & 0.28 & 1300 & 15 & 1 & 0.075 & RH, RR & C/X & Double RH. Radio bridge. RR in A1758S. Revived fossil plasma \\
PSZ2 G107.11-39.50 & 359.7704 & 21.7518 & 0.533 & 6.93 & 0.67 & 1114 & 36 & 1 & 0.102 & U & --- & --- \\
PSZ2 G107.39-31.48 & 357.6390 & 29.5399 & 0.150 & 3.45 & 0.45 & 1019 & 45 & 1 & 0.104 & NDE & --- & --- \\
PSZ2 G107.67-39.78 & 0.3019 & 21.5932 & 0.415 & 5.73 & 0.75 & 1095 & 48 & 2 & 0.101 & U & --- & --- \\
PSZ2 G108.24+58.11 & 207.2301 & 57.3469 & 0.322 & 3.85 & 0.53 & 994 & 46 & 1 & 0.183 & U & --- & --- \\
PSZ2 G108.27+48.66 & 216.7773 & 65.6528 & 0.674 & 4.93 & 0.49 & 940 & 32 & 1 & 0.134 & cRH & --- & New cRH \\
PSZ2 G109.14-28.02 & 358.2865 & 33.2800 & 0.457 & 6.92 & 0.62 & 1147 & 34 & 3 & 0.096 & N/A & --- & --- \\
PSZ2 G109.22-44.01 & 2.5556 & 17.7559 & 0.173 & 3.26 & 0.48 & 993 & 49 & 2 & 0.190 & cRR & --- & New cRR \\
PSZ2 G109.97+52.84 & 209.9356 & 62.5279 & 0.326 & 4.81 & 0.38 & 1069 & 28 & 1 & 0.067 & RH & C & New RH \\
PSZ2 G111.75+70.37 & 198.2642 & 46.2812 & 0.183 & 4.34 & 0.33 & 1088 & 27 & 1 & 0.076 & RH, RR & C/X & RR in the NE \\
PSZ2 G112.07-39.86 & 3.8730 & 22.2454 &  &  &  &  &  & 2 & 0.135 & NDE & --- & --- \\
PSZ2 G112.35-32.86 & 2.6884 & 29.1673 & 0.348 & 5.50 & 0.68 & 1108 & 46 & 2 & 0.166 & NDE & X & --- \\
PSZ2 G112.48+56.99 & 203.9932 & 59.2210 & 0.070 & 2.99 & 0.15 & 998 & 17 & 1 & 0.058 & RH & C & New RH \\
PSZ2 G112.54+59.53 & 202.4759 & 56.8123 & 0.830 & 5.76 & 0.66 & 930 & 36 & 1 & 0.071 & NDE & --- & Redshift updated from Zohren et al. (2019) \\
PSZ2 G113.27+48.39 & 209.7444 & 67.4431 &  &  &  &  &  & 1 & 0.072 & NDE & --- & --- \\
PSZ2 G113.29-29.69 & 2.9363 & 32.4325 & 0.107 & 3.71 & 0.27 & 1060 & 25 & 2 & 0.114 & U & C/X & --- \\
PSZ2 G113.91-37.01 & 4.9004 & 25.2965 & 0.371 & 7.58 & 0.55 & 1223 & 30 & 1 & 0.122 & RH, RR & C/X & New RH and RR. Double RR \\
PSZ2 G114.14+58.96 & 201.3065 & 57.5834 & 0.116 & 2.17 & 0.30 & 884 & 41 & 2 & 0.069 & NDE & --- & Possible revived fossil plasma \\
PSZ2 G114.31+64.89 & 198.7658 & 51.8329 & 0.284 & 6.76 & 0.37 & 1216 & 22 & 1 & 0.071 & RH & C/X & --- \\
PSZ2 G114.39-20.98 & 2.2522 & 41.1782 & 0.154 & 3.81 & 0.35 & 1053 & 32 & 1 & 0.187 & NDE & --- & --- \\
PSZ2 G114.79-33.71 & 5.1456 & 28.6657 & 0.094 & 3.82 & 0.22 & 1075 & 21 & 2 & 0.133 & NDE & C/X & --- \\
PSZ2 G114.83+57.25 & 201.4457 & 59.3305 & 0.170 & 3.27 & 0.30 & 995 & 31 & 1 & 0.076 & NDE & --- & --- \\
PSZ2 G114.90-34.35 & 5.3526 & 28.0504 & 0.095 & 2.47 & 0.32 & 929 & 41 & 2 & 0.140 & U & --- & --- \\
PSZ2 G114.99+70.36 & 196.7286 & 46.5257 & 0.226 & 5.70 & 0.35 & 1174 & 24 & 2 & 0.086 & U & C & Complex radio emission \\
PSZ2 G115.58-44.56 & 7.3620 & 17.9947 & 0.170 & 4.32 & 0.40 & 1091 & 34 & 1 & 0.100 & NDE & --- & --- \\
PSZ2 G115.67-27.57 & 5.0172 & 34.8529 & 0.457 & 5.31 & 0.75 & 1050 & 50 & 1 & 0.100 & cRH & --- & --- \\
PSZ2 G116.32-36.33 & 6.9294 & 26.2373 & 0.367 & 5.31 & 0.63 & 1087 & 43 & 3 & 0.128 & N/A & C/X & --- \\
PSZ2 G116.50-44.47 & 8.0345 & 18.1536 & 0.396 & 7.61 & 0.60 & 1213 & 32 & 1 & 0.111 & RH*, RR & X & New RH* and RR \\
PSZ2 G118.34+68.79 & 195.3484 & 48.2419 & 0.255 & 3.77 & 0.49 & 1012 & 44 & 1 & 0.071 & cRH* & --- & --- \\
PSZ2 G118.49+48.17 & 201.0202 & 68.6690 & 0.320 & 3.68 & 0.41 & 980 & 37 & 1 & 0.077 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G118.92+52.38 & 198.5514 & 64.5643 & 0.220 & 4.39 & 0.29 & 1078 & 24 & 1 & 0.059 & U & --- & --- \\
PSZ2 G119.92+59.12 & 195.7642 & 57.9334 & 0.196 & 3.44 & 0.33 & 1002 & 32 & 1 & 0.072 & U & --- & --- \\
PSZ2 G120.08-44.41 & 10.7148 & 18.4071 & 0.267 & 4.65 & 0.64 & 1080 & 49 & 2 & 0.218 & NDE & --- & --- \\
PSZ2 G121.03+57.02 & 194.9266 & 60.0741 & 0.344 & 5.69 & 0.43 & 1123 & 28 & 1 & 0.089 & RR, U & C & New RR. U emission in the center \\
PSZ2 G121.13+49.64 & 195.8869 & 67.4415 & 0.221 & 3.17 & 0.36 & 967 & 37 & 1 & 0.091 & NDE & X & --- \\
PSZ2 G121.77+51.75 & 194.5723 & 65.3600 & 0.233 & 3.98 & 0.41 & 1038 & 35 & 1 & 0.056 & NDE & --- & --- \\
PSZ2 G121.87-45.97 & 12.0892 & 16.8876 &  &  &  &  &  & 2 & 0.237 & NDE & --- & --- \\
PSZ2 G122.30+54.52 & 193.6463 & 62.5963 & 0.318 & 4.53 & 0.45 & 1050 & 35 & 1 & 0.094 & NDE & --- & --- \\
PSZ2 G122.47-38.41 & 12.4689 & 24.4527 & 0.082 & 2.52 & 0.31 & 939 & 38 & 2 & 0.115 & U & --- & --- \\
PSZ2 G122.89-36.82 & 12.8246 & 26.0510 & 0.346 & 5.57 & 0.73 & 1114 & 49 & 1 & 0.083 & NDE & --- & --- \\
PSZ2 G123.00-35.52 & 12.9231 & 27.3461 & 0.380 & 6.47 & 0.65 & 1156 & 39 & 2 & 0.077 & RH* & X & New RH* \\
PSZ2 G123.66+67.25 & 192.4223 & 49.8718 & 0.284 & 4.38 & 0.51 & 1053 & 41 & 1 & 0.064 & NDE & C & --- \\
PSZ2 G124.20-36.48 & 14.0018 & 26.3784 & 0.197 & 7.65 & 0.36 & 1308 & 20 & 3 & 0.113 & N/A & C/X & --- \\
PSZ2 G125.30-27.99 & 15.4081 & 34.8346 & 0.223 & 5.02 & 0.55 & 1126 & 41 & 1 & 0.111 & U & --- & --- \\
PSZ2 G125.71+53.86 & 189.2251 & 63.1843 & 0.302 & 6.55 & 0.33 & 1195 & 20 & 3 & 0.072 & N/A & C/X & --- \\
PSZ2 G126.20-33.17 & 16.0136 & 29.6172 & 0.358 & 5.45 & 0.74 & 1101 & 50 & 1 & 0.123 & NDE & --- & --- \\
PSZ2 G126.28+65.62 & 190.6409 & 51.4447 & 0.820 & 5.54 & 0.66 & 922 & 37 & 1 & 0.055 & U & --- & Redshift updated from Burenin et al. (2018) \\
PSZ2 G126.57+51.61 & 187.4359 & 65.3561 & 0.815 & 6.47 & 0.61 & 973 & 31 & 1 & 0.066 & NDE & C & Redshift updated from Burenin et al. (2018) \\
PSZ2 G126.61-37.63 & 16.0784 & 25.1450 & 0.166 & 3.84 & 0.50 & 1050 & 46 & 3 & 0.169 & N/A & X & --- \\
PSZ2 G126.72-21.03 & 17.6030 & 41.6924 & 0.220 & 4.11 & 0.57 & 1055 & 49 & 1 & 0.110 & NDE & --- & Redshift updated from Burenin et al. (2018) \\
PSZ2 G127.44-34.74 & 17.0569 & 27.9786 & 0.249 & 4.90 & 0.71 & 1106 & 54 & 2 & 0.131 & NDE & --- & --- \\
PSZ2 G127.50-30.52 & 17.5164 & 32.1829 & 0.353 & 5.29 & 0.67 & 1092 & 46 & 1 & 0.107 & NDE & X & --- \\
PSZ2 G128.15-24.71 & 18.8768 & 37.9135 & 0.263 & 4.48 & 0.60 & 1068 & 48 & 1 & 0.069 & NDE & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G129.99-22.42 & 21.3891 & 39.9803 &  &  &  &  &  & 1 & 0.081 & NDE & --- & --- \\
PSZ2 G130.25-26.50 & 20.9524 & 35.9025 & 0.216 & 4.49 & 0.50 & 1088 & 40 & 2 & 0.102 & NDE & --- & --- \\
PSZ2 G131.27-25.82 & 22.2049 & 36.4447 &  &  &  &  &  & 1 & 0.141 & NDE & --- & --- \\
PSZ2 G132.54-42.16 & 20.4346 & 20.1398 & 0.194 & 3.99 & 0.51 & 1054 & 45 & 1 & 0.152 & NDE & X & --- \\
PSZ2 G133.59+50.68 & 176.7040 & 65.0891 & 0.529 & 5.16 & 0.57 & 1011 & 37 & 1 & 0.076 & RH* & X & New RH* \\
PSZ2 G133.60+69.04 & 187.2235 & 47.6123 & 0.254 & 5.88 & 0.40 & 1173 & 27 & 1 & 0.069 & RH & C & Possible revived fossil plasma \\
PSZ2 G133.92-42.73 & 21.4010 & 19.4054 & 0.636 & 7.24 & 0.96 & 1085 & 48 & 1 & 0.116 & NDE & --- & Redshift updated from Burenin (2017) \\
PSZ2 G134.26-44.28 & 21.3587 & 17.8353 &  &  &  &  &  & 1 & 0.152 & NDE & --- & --- \\
PSZ2 G134.59+53.38 & 177.7969 & 62.3578 & 0.345 & 4.45 & 0.54 & 1034 & 42 & 2 & 0.080 & NDE & --- & --- \\
PSZ2 G134.70+48.91 & 173.3085 & 66.3869 & 0.116 & 3.40 & 0.22 & 1027 & 22 & 2 & 0.107 & NDE & C/X & --- \\
PSZ2 G135.06+54.39 & 178.0903 & 61.3191 & 0.317 & 5.41 & 0.42 & 1115 & 29 & 1 & 0.065 & NDE & --- & --- \\
PSZ2 G135.17+65.43 & 184.8205 & 50.9217 & 0.544 & 6.01 & 0.60 & 1057 & 35 & 2 & 0.071 & RH, RR & C & --- \\
PSZ2 G135.19+57.88 & 180.5387 & 58.0593 & 0.103 & 2.21 & 0.23 & 893 & 31 & 3 & 0.133 & N/A & C & --- \\
PSZ2 G136.31+54.67 & 176.9598 & 60.7656 & 0.477 & 5.98 & 0.51 & 1084 & 31 & 1 & 0.069 & NDE & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G136.33-44.53 & 22.8257 & 17.3003 &  &  &  &  &  & 1 & 0.197 & NDE & --- & --- \\
PSZ2 G136.64-25.03 & 28.2988 & 36.1888 & 0.016 & 1.12 & 0.11 & 732 & 24 & 2 & 0.125 & NDE & C/X & --- \\
PSZ2 G136.92+59.46 & 180.0852 & 56.2524 & 0.065 & 1.81 & 0.16 & 846 & 25 & 2 & 0.103 & U & X & --- \\
PSZ2 G137.24+53.93 & 175.2772 & 61.1942 & 0.470 & 7.00 & 0.48 & 1146 & 26 & 1 & 0.063 & NDE & --- & Redshift updated from Boada et al. (2019) \\
PSZ2 G137.58+53.88 & 174.8622 & 61.1503 &  &  &  &  &  & 1 & 0.084 & NDE & --- & --- \\
PSZ2 G137.74-27.08 & 28.7835 & 33.9443 & 0.087 & 2.83 & 0.28 & 975 & 32 & 2 & 0.123 & NDE & X & Possible revived fossil plasma \\
PSZ2 G138.32-39.82 & 25.5157 & 21.5330 & 0.280 & 5.98 & 0.56 & 1169 & 37 & 1 & 0.138 & RH & C & --- \\
PSZ2 G139.00+50.92 & 170.0451 & 63.2596 & 0.784 & 5.90 & 0.70 & 955 & 38 & 1 & 0.077 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G139.18+56.37 & 175.5928 & 58.5227 & 0.322 & 6.87 & 0.38 & 1205 & 22 & 1 & 0.068 & RH & C/X & --- \\
PSZ2 G139.72-17.13 & 34.9806 & 42.8317 & 0.155 & 3.61 & 0.44 & 1033 & 42 & 1 & 0.153 & NDE & --- & Redshift updated from Streblyanska et al. (2019) \\
PSZ2 G141.05-32.61 & 30.0905 & 27.8208 & 0.554 & 6.92 & 0.77 & 1104 & 41 & 2 & 0.124 & cRH & --- & New cRH \\
PSZ2 G141.98+69.31 & 183.2387 & 46.3648 & 0.713 & 5.29 & 0.68 & 948 & 40 & 1 & 0.087 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G143.26+65.24 & 179.8427 & 49.7742 & 0.363 & 7.65 & 0.43 & 1230 & 23 & 1 & 0.061 & RH & C/X & --- \\
PSZ2 G143.44+53.66 & 168.7489 & 59.4513 & 0.366 & 5.31 & 0.57 & 1088 & 39 & 2 & 0.067 & U & --- & Possible revived fossil plasma \\
PSZ2 G143.62+42.61 & 150.8432 & 67.1371 & 0.206 & 4.95 & 0.34 & 1127 & 26 & 1 & 0.087 & NDE & --- & --- \\
PSZ2 G144.23-18.19 & 39.7214 & 40.1886 &  &  &  &  &  & 1 & 0.096 & cRH & --- & New cRH \\
PSZ2 G144.33+62.85 & 177.3062 & 51.6086 & 0.132 & 2.66 & 0.35 & 940 & 42 & 1 & 0.063 & NDE & --- & --- \\
PSZ2 G144.84-35.16 & 32.4230 & 24.3554 &  &  &  &  &  & 1 & 0.092 & NDE & --- & --- \\
PSZ2 G144.99-24.64 & 37.1891 & 34.0270 & 0.190 & 4.25 & 0.50 & 1077 & 42 & 2 & 0.097 & cRR, U & --- & New cRR. U emission located in the center of the images \\
PSZ2 G145.25+50.84 & 163.3572 & 60.8620 &  &  &  &  &  & 1 & 0.073 & NDE & --- & --- \\
PSZ2 G145.65+59.30 & 173.1514 & 54.2102 & 0.347 & 4.73 & 0.61 & 1054 & 46 & 2 & 0.076 & U & X & --- \\
PSZ2 G146.13+40.97 & 144.7845 & 66.4371 & 0.342 & 4.70 & 0.65 & 1054 & 49 & 1 & 0.076 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G146.82+40.97 & 144.1849 & 65.9752 & 0.259 & 4.49 & 0.27 & 1071 & 21 & 1 & 0.070 & NDE & --- & --- \\
PSZ2 G147.17+42.67 & 147.4525 & 64.9221 & 0.460 & 5.65 & 0.72 & 1071 & 46 & 1 & 0.078 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G147.88+53.24 & 164.3924 & 58.0187 & 0.600 & 6.47 & 0.60 & 1060 & 33 & 1 & 0.065 & cRH & --- & --- \\
PSZ2 G148.36+75.23 & 184.6185 & 40.2211 & 0.304 & 4.75 & 0.50 & 1073 & 38 & 1 & 0.075 & RH & C & New RH \\
PSZ2 G149.22+54.18 & 164.6039 & 56.7926 & 0.137 & 5.87 & 0.22 & 1222 & 15 & 2 & 0.083 & RH & C & --- \\
PSZ2 G149.75+34.68 & 127.7147 & 65.8623 & 0.182 & 8.86 & 0.32 & 1381 & 17 & 1 & 0.069 & RH & C/X & --- \\
PSZ2 G150.24+48.72 & 155.8514 & 59.8085 & 0.205 & 3.56 & 0.42 & 1010 & 40 & 1 & 0.066 & NDE & --- & --- \\
PSZ2 G150.56+46.67 & 152.1830 & 60.7778 & 0.398 & 5.21 & 0.62 & 1068 & 42 & 1 & 0.061 & cRH & --- & --- \\
PSZ2 G150.56+58.32 & 168.7952 & 53.3275 & 0.470 & 7.55 & 0.51 & 1175 & 26 & 2 & 0.075 & RH & C/X & --- \\
PSZ2 G151.19+48.27 & 154.4084 & 59.5510 & 0.289 & 5.08 & 0.47 & 1103 & 34 & 2 & 0.059 & RH, RR & C/X & --- \\
PSZ2 G151.62+54.78 & 163.7128 & 55.3610 & 0.486 & 5.37 & 0.72 & 1042 & 47 & 3 & 0.155 & N/A & --- & --- \\
PSZ2 G152.33+81.28 & 187.6699 & 34.6290 & 0.333 & 5.36 & 0.55 & 1105 & 38 & 2 & 0.084 & NDE & --- & Possible revived fossil plasma \\
PSZ2 G152.40+75.00 & 183.3147 & 39.8577 & 0.453 & 5.14 & 0.70 & 1040 & 47 & 1 & 0.074 & NDE & --- & Redshift updated from Streblyanska et al. (2018) \\
PSZ2 G152.47+42.11 & 142.4647 & 61.6579 & 0.900 & 6.58 & 0.77 & 946 & 37 & 1 & 0.096 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G153.29+36.56 & 130.6776 & 62.6758 & 0.650 & 6.32 & 1.27 & 1031 & 68 & 1 & 0.077 & NDE & --- & --- \\
PSZ2 G153.56+36.82 & 131.1332 & 62.4117 &  &  &  &  &  & 1 & 0.068 & NDE & --- & --- \\
PSZ2 G153.57+36.26 & 129.9422 & 62.5148 & 0.132 & 3.37 & 0.39 & 1018 & 39 & 1 & 0.077 & NDE & --- & --- \\
PSZ2 G153.68+36.96 & 131.3866 & 62.2867 &  &  &  &  &  & 1 & 0.070 & NDE & --- & --- \\
PSZ2 G153.80+33.79 & 124.5597 & 62.6820 &  &  &  &  &  & 1 & 0.070 & NDE & --- & --- \\
PSZ2 G154.13+40.19 & 137.8076 & 61.1324 & 0.290 & 5.47 & 0.45 & 1131 & 31 & 1 & 0.087 & cRH & --- & New cRH \\
PSZ2 G155.80+70.40 & 178.4833 & 42.8600 & 0.333 & 4.42 & 0.56 & 1036 & 44 & 1 & 0.071 & NDE & --- & Possible revived fossil plasma \\
PSZ2 G156.26+59.64 & 167.1024 & 50.2811 & 0.588 & 6.77 & 0.60 & 1081 & 32 & 2 & 0.096 & cRH & --- & --- \\
PSZ2 G157.63+78.02 & 184.3872 & 36.7167 & 0.377 & 5.56 & 0.57 & 1100 & 38 & 2 & 0.072 & U & --- & --- \\
PSZ2 G159.86+42.57 & 139.8791 & 56.3460 & 0.270 & 4.61 & 0.57 & 1076 & 44 & 1 & 0.080 & NDE & --- & --- \\
PSZ2 G160.83+81.66 & 186.7250 & 33.5703 & 0.888 & 5.70 & 0.66 & 906 & 35 & 1 & 0.087 & RH & C/X & --- \\
PSZ2 G160.94+44.85 & 143.3681 & 54.9523 &  &  &  &  &  & 1 & 0.082 & NDE & --- & --- \\
PSZ2 G163.61+34.30 & 124.7099 & 54.5333 & 0.596 & 5.76 & 0.74 & 1021 & 44 & 2 & 0.079 & cRH* & --- & New cRH* \\
PSZ2 G163.69+53.52 & 155.5975 & 50.1197 & 0.158 & 4.73 & 0.31 & 1130 & 24 & 2 & 0.090 & U & C & --- \\
PSZ2 G163.87+48.54 & 148.2005 & 51.8883 & 0.214 & 3.62 & 0.43 & 1013 & 41 & 1 & 0.059 & NDE & C & --- \\
PSZ2 G164.65+46.37 & 144.5898 & 52.0336 & 0.342 & 6.01 & 0.55 & 1144 & 35 & 1 & 0.070 & RH & C & New RH \\
PSZ2 G165.06+54.13 & 155.9404 & 49.1327 & 0.144 & 4.94 & 0.28 & 1152 & 22 & 1 & 0.078 & RH & C & --- \\
PSZ2 G165.46+66.15 & 170.9186 & 43.0135 & 0.196 & 3.70 & 0.42 & 1027 & 39 & 1 & 0.108 & RR & C & Double RR \\
PSZ2 G165.68+44.01 & 140.5859 & 51.8876 & 0.210 & 3.76 & 0.50 & 1027 & 46 & 1 & 0.072 & NDE & --- & --- \\
PSZ2 G165.76+31.15 & 119.5415 & 52.5986 & 0.259 & 4.43 & 0.66 & 1066 & 54 & 2 & 0.131 & NDE & --- & --- \\
PSZ2 G165.95+41.01 & 135.7227 & 52.2021 & 0.062 & 1.79 & 0.26 & 843 & 40 & 1 & 0.079 & NDE & C/X & --- \\
PSZ2 G166.09+43.38 & 139.4836 & 51.7221 & 0.217 & 6.85 & 0.32 & 1251 & 20 & 1 & 0.074 & RH & C/X & --- \\
PSZ2 G166.62+42.13 & 137.3948 & 51.5489 & 0.232 & 5.34 & 0.40 & 1145 & 28 & 1 & 0.081 & RH, RR & C & RH contaminated by RR emission. Multiple RR \\
PSZ2 G168.33+69.73 & 174.0505 & 40.1032 & 0.288 & 4.79 & 0.50 & 1083 & 37 & 1 & 0.102 & U & C & Possible revived fossil plasma \\
PSZ2 G169.62+33.84 & 124.1776 & 49.5502 & 0.347 & 5.92 & 0.63 & 1136 & 40 & 3 & 0.125 & N/A & --- & --- \\
PSZ2 G170.26+73.90 & 178.0167 & 37.2537 & 0.165 & 3.12 & 0.42 & 981 & 45 & 2 & 0.094 & U & --- & --- \\
PSZ2 G170.98+39.45 & 132.7602 & 48.5104 & 0.538 & 8.08 & 0.68 & 1170 & 33 & 2 & 0.092 & U & C & --- \\
PSZ2 G172.63+35.15 & 126.3699 & 47.1532 & 0.127 & 3.90 & 0.34 & 1071 & 31 & 1 & 0.180 & RH & C & New RH \\
PSZ2 G172.74+65.30 & 167.9029 & 40.8574 & 0.079 & 2.45 & 0.21 & 932 & 27 & 2 & 0.105 & U & C/X & Possible revived fossil plasma \\
PSZ2 G175.60+35.47 & 127.0828 & 44.7549 & 0.145 & 3.08 & 0.40 & 983 & 43 & 2 & 0.109 & U & C & --- \\
PSZ2 G176.27+37.54 & 130.0378 & 44.3618 & 0.567 & 6.14 & 0.86 & 1056 & 50 & 2 & 0.091 & RH & C & --- \\
PSZ2 G177.03+32.64 & 123.3526 & 43.2651 & 0.511 & 6.07 & 0.76 & 1075 & 45 & 1 & 0.120 & NDE & --- & Redshift updated from Aguado-Barahona et al. (2019) \\
PSZ2 G178.00+42.32 & 136.6840 & 43.1361 & 0.237 & 3.97 & 0.54 & 1036 & 47 & 1 & 0.073 & NDE & --- & --- \\
PSZ2 G178.94+56.00 & 154.9481 & 41.0098 & 0.092 & 2.23 & 0.30 & 899 & 40 & 1 & 0.074 & NDE & --- & --- \\
PSZ2 G179.09+60.12 & 160.1864 & 39.9592 & 0.137 & 3.84 & 0.33 & 1061 & 30 & 1 & 0.093 & RH & C/X & New RH \\
PSZ2 G180.60+76.65 & 179.3110 & 33.6110 & 0.214 & 6.30 & 0.34 & 1218 & 22 & 2 & 0.094 & NDE & C & --- \\
PSZ2 G180.88+31.04 & 121.9739 & 39.7755 & 0.365 & 5.99 & 0.70 & 1133 & 44 & 3 & 0.112 & N/A & X & --- \\
PSZ2 G181.06+48.47 & 144.8501 & 40.7576 & 0.240 & 4.23 & 0.49 & 1057 & 41 & 1 & 0.066 & RR & C & New RR. Double RR \\
PSZ2 G182.59+55.83 & 154.2574 & 39.0280 & 0.206 & 5.83 & 0.34 & 1191 & 23 & 3 & 0.095 & N/A & C/X & --- \\
PSZ2 G183.30+34.98 & 127.4335 & 38.4548 & 0.392 & 6.56 & 0.64 & 1156 & 38 & 2 & 0.097 & cRH, U & --- & New cRH. U emisssion located in the E \\
PSZ2 G183.90+42.99 & 137.6963 & 38.8112 & 0.561 & 6.95 & 0.74 & 1102 & 39 & 1 & 0.096 & RH & X & --- \\
PSZ2 G184.24+43.69 & 138.6019 & 38.6019 & 0.397 & 5.41 & 0.63 & 1082 & 42 & 1 & 0.077 & NDE & --- & --- \\
PSZ2 G184.68+28.91 & 120.2399 & 36.0972 & 0.288 & 5.50 & 0.52 & 1134 & 36 & 1 & 0.088 & RH & C/X & New RH \\
PSZ2 G185.08+34.02 & 126.5397 & 36.8505 & 0.365 & 5.41 & 0.66 & 1095 & 44 & 1 & 0.111 & NDE & --- & --- \\
PSZ2 G186.37+37.26 & 130.7485 & 36.3528 & 0.282 & 11.00 & 0.37 & 1431 & 16 & 1 & 0.107 & RH & C/X & --- \\
PSZ2 G186.61+62.94 & 162.6646 & 35.8429 & 0.509 & 5.68 & 0.65 & 1052 & 40 & 1 & 0.067 & cRH & --- & New cRH \\
PSZ2 G186.99+38.65 & 132.5385 & 36.0766 & 0.378 & 6.84 & 0.52 & 1178 & 30 & 2 & 0.092 & RH, RR & C & New RH and RR \\
PSZ2 G187.53+21.92 & 113.0646 & 31.6261 & 0.171 & 5.17 & 0.39 & 1158 & 29 & 2 & 0.160 & U & C/X & --- \\
PSZ2 G187.74+20.66 & 111.7531 & 31.0220 & 0.193 & 4.29 & 0.50 & 1080 & 42 & 3 & 0.218 & N/A & --- & --- \\
PSZ2 G189.23+20.55 & 112.1961 & 29.6730 & 0.398 & 5.46 & 0.74 & 1085 & 50 & 2 & 0.147 & NDE & --- & --- \\
PSZ2 G189.31+59.24 & 157.9544 & 35.0406 & 0.126 & 3.24 & 0.31 & 1007 & 32 & 1 & 0.103 & RH & C & New RH. Revived fossil plasma \\
PSZ2 G190.61+66.46 & 166.5376 & 33.5720 & 0.488 & 5.55 & 0.65 & 1053 & 41 & 1 & 0.077 & RH, RR & C & New RH and RR \\
PSZ2 G191.57+58.88 & 157.4152 & 33.9099 &  &  &  &  &  & 1 & 0.107 & NDE & --- & --- \\
PSZ2 G192.18+56.12 & 154.0911 & 33.6604 & 0.124 & 3.62 & 0.30 & 1045 & 29 & 1 & 0.089 & RH & C/X & New RH \\
PSZ2 G192.77+33.14 & 127.1718 & 30.4022 & 0.050 & 1.66 & 0.20 & 825 & 34 & 2 & 0.116 & cRH & --- & New cRH \\
PSZ2 G192.90+29.63 & 123.3039 & 29.3652 & 0.360 & 5.17 & 0.76 & 1080 & 53 & 1 & 0.119 & cRH & --- & New cRH \\
PSZ2 G193.63+54.85 & 152.5729 & 32.8307 & 0.292 & 5.19 & 0.52 & 1110 & 37 & 2 & 0.134 & U & X & --- \\
PSZ2 G194.98+54.12 & 151.7502 & 32.0212 & 0.375 & 5.66 & 0.66 & 1108 & 43 & 2 & 0.120 & U & C & --- \\
PSZ2 G195.24+29.34 & 123.6579 & 27.3366 & 0.284 & 4.94 & 0.62 & 1095 & 46 & 2 & 0.113 & U & --- & --- \\
PSZ2 G195.60+44.06 & 140.0993 & 30.5038 & 0.295 & 6.13 & 0.48 & 1172 & 31 & 2 & 0.105 & NDE & C/X & --- \\
PSZ2 G197.13+33.46 & 128.6143 & 26.9731 & 0.456 & 5.87 & 0.69 & 1086 & 43 & 1 & 0.109 & U & --- & --- \\
PSZ2 G198.46+46.01 & 142.7118 & 28.8476 & 0.299 & 5.55 & 0.54 & 1132 & 37 & 1 & 0.088 & cRR, U & --- & New cRR \\
PSZ2 G199.61+53.41 & 151.2012 & 29.2311 & 0.371 & 5.54 & 0.59 & 1101 & 39 & 1 & 0.095 & NDE & --- & --- \\
PSZ2 G199.75+46.59 & 143.5387 & 28.0764 & 0.553 & 5.91 & 0.76 & 1048 & 45 & 2 & 0.098 & NDE & --- & --- \\
PSZ2 G200.06+77.22 & 178.5581 & 29.2431 & 0.361 & 4.62 & 0.61 & 1041 & 46 & 3 & 0.130 & N/A & --- & --- \\
PSZ2 G202.66+66.98 & 166.8142 & 28.7965 & 0.483 & 5.28 & 0.70 & 1038 & 46 & 1 & 0.115 & NDE & --- & Redshift updated from Streblyanska et al. (2018) \\
PSZ2 G203.22+66.40 & 166.1721 & 28.5492 & 0.580 & 5.89 & 0.71 & 1036 & 42 & 3 & 0.130 & N/A & --- & --- \\
PSZ2 G205.90+73.76 & 174.5534 & 27.9203 & 0.447 & 7.39 & 0.55 & 1177 & 29 & 1 & 0.101 & RH, RR & C & New RH and RR. Double RR \\
